Multiple conditional randomization tests for lagged and spillover treatment effects

We consider the problem of constructing multiple independent conditional randomization tests using a single dataset. Because the tests are independent, the randomization p-values can be interpreted individually and combined using standard methods for multiple testing. We give a simple, sequential construction of such tests, and then discuss its application to three problems: Rosenbaum's evidence factors for observational studies, lagged treatment effect in stepped-wedge trials, and spillover effect in randomized trials with interference. We compare the proposed approach with some existing methods using simulated and real datasets. Finally, we establish a more general sufficient condition for independent conditional randomization tests.

==> 4_Example.tex <==

\section{Conditional randomization tests in the literature}
\label{sec:examples}

Next, we apply the general theory in
\Cref{sec:single-crt,sec:multiple-crt} to better understand some
(conditional) randomization tests that have been proposed in the
literature.

\subsection{Permutation tests for treatment effect}
\label{sec:permutation-tests}

Permutation test is the most well known form of conditional
randomization tests. In a permutation test, the p-value is obtained
by calculating all possible values of the test statistics under all
possible permutations of the observed data points. In our setup,
this amounts to use the conditioning sets (suppose $\bm Z$ is a vector
of length $N$)
\begin{equation}
  \label{eq:sz-permutation}
  \mathcal{S}_{\bm z} = \{(z_{\sigma(1)},\dotsc,z_{\sigma(N)}):\text{$\sigma$
    is a permutation of $[N]$}\}.
\end{equation}
In view of \Cref{prop:condition-on-function}, permutation test is a
CRT that conditions on the order statistics of $\bm Z$.
In permutation tests, the treatment assignments are typically assumed
to be exchangeable,
\[
  (Z_1,\dotsc,Z_N) \overset{d}{=} (Z_{\sigma(1)}, \dotsc,
  Z_{\sigma(N)})~\text{for all permutations $\sigma$ of $[N]$},
\]
so each permutation of $\bm Z$ has the same probability of being
realized under the treatment assignment mechanism
$\pi(\cdot)$. See
\cite{kalbfleisch78_likel_method_nonpar_tests} for an alternative
formulation of rank-based tests based on marginal and conditional
likelihoods. Examples of exchangeable assignments include repeated
Bernoulli trials and simple random sampling with or without
replacement (let $Z_i$ be the number of times unit $i$ is
sampled). Exchangeability makes it straightforward to compute the
p-value \eqref{eq:p-value}, as $\bm Z^{*}$ is uniformly distributed
over $\mathcal{S}_{\bm Z}$ if $\bm Z$ has
distinct elements. In this sense, our assumption that the assignment
distribution of $\bm Z$ is known (\Cref{assump:randomization}) is more
general than exchangeability. See \cite{roach2018permutation} for
some recent development on generalized permutation tests in
non-exchangeable models.

Notice that in permutation tests, the invariance of $\mathcal{S}_{\bm
  z}$ in \Cref{lem:same-st} is satisfied because the permutation group
is closed under composition, that is, the composition of two
permutations of $[N]$ is still a permutation of $[N]$. This property
can be violated when the test conditions on additional
events. Southworth et al.\ \cite{southworth2009properties} gives a counterexample in
which $\bm Z$ is randomized uniformly over
\[
  \mathcal{Z} = \{\bm z \in
  \{0,1\}^N: \bm z^T \bm 1 = N/2\},
\]
so exactly half of the units are treated. They consider the ``balanced
permutation test'' in \citep[Section 6]{efron2001empirical} that uses the
following conditioning set
\begin{equation}
  \label{eq:balanced-permutation}
  \mathcal{S}_{\bm z} = \{\bm z^{*}:
  \text{$\bm z^{*}$ is a permutation of $\bm z$ and } \bm z^T \bm z^{*}
  = N/4\}.
\end{equation}
Southworth et al.\ \cite{southworth2009properties} showed that the standard theory
for permutation tests in \citep{lehmann2006testing} does not
establish the validity of the balanced permutation tests, because
$\mathcal{S}_{\bm z}$ is not a group under
balanced permutations (nor is $\mathcal{S}_{\bm z} \cup \{\bm
z\}$). They also provided numerical examples in which
the balanced permutation test has an inflated type I error.

With the general theory in \Cref{sec:single-crt} in mind, we see that
\eqref{eq:balanced-permutation} clearly does not satisfy the
invariance property in \Cref{lem:same-st}. Moreover, a group
structure is not necessary in the construction of a valid
randomization test in \Cref{sec:single-crt}. The crucial algebraic structure is that
$\mathcal{R} = \{\mathcal{S}_{\bm z}:\bm z \in \mathcal{Z}\}$ must be a
partition of $\mathcal{Z}$, or equivalently that the conditioning set
$\mathcal{S}_{\bm z}$ must be defined by an equivalence relation. This
is clearly not satisfied by \eqref{eq:balanced-permutation}.

\subsection{Permutation tests for independence}
\label{sec:tests-cond-indep}

Randomization tests are frequently used to test the independence of random
variables. % In fact, any exact hypothesis test must be a permutation
% test, because the vector of order statistics is a complete suffcient
% statistics; see \citep[Theorem 5.8.1]{lehmann2006testing} or
% \citep[Theorem 3.2.1.1]{hajek1999theory}.
In this problem, it is typically assumed that we observe
independent and identically distributed random variables
$(Z_1,Y_1),\dotsc,(Z_n,Y_n)$ and would like to test the null
hypothesis that $Z_1$ and $Y_1$ are independent. In the classical
treatment of this problem \citep{lehmann2006testing,hajek1999theory},
the key idea is to establish the following \emph{permutation
  principle}:
\[
  (Z_1,\dotsc,Z_N,Y_1,\dotsc,Y_N) \overset{d}{=}
  (Z_{\sigma(1)},\dotsc,Z_{\sigma(N)},Y_1,\dotsc,Y_N)~\text{for all
    permutations $\sigma$ of $[N]$}.
\]
Let $\bm Z = (Z_1, \dotsc, Z_N)$, $\bm Y = (Y_1,\dotsc,Y_N)$, and
$\bm Z_{\sigma} = (Z_{\sigma(1)}, \dotsc, Z_{\sigma(N)})$. Then given
a test statistic $T(\bm Z, \bm Y)$, independence is rejected if the
following p-value is less than the significance level (recall that
there are $N!$ permutations of $[N]$):
\begin{equation}
  \label{eq:p-value-permutation}
  P(\bm Z, \bm Y) = \frac{1}{N!} \sum_{\sigma} 1_{\{T(\bm Z_{\sigma},
    \bm Y) \leq T(\bm Z, \bm Y)\}}.
\end{equation}
We are using the same notation $P(\bm Z, \bm Y)$ for the
p-value of this permutation test in \eqref{eq:p-value-permutation},
because they are indeed identical. It might seem that the permutation
test is solving a different problem
from testing a causal null hypothesis---after all, no
counterfactuals are involved in testing independence. In fact,
Lehmann \cite{lehmann1975nonparametrics} referred to the causal inference
problem as the \emph{randomization model} and the independence testing
problem as the \emph{population
  model}. Ernst \cite{ernst2004permutation} argued that the reasoning
behind these two models is different.

However, a statistical test not only explicitly tests the null hypothesis $H_0$
but also implicitly tests any assumptions needed to set up the
problem. Therefore, the CRT described in \Cref{sec:single-crt} tests
not only a partially sharp null hypothesis about the causal effect
but also the assumption that the treatment is randomized
(\Cref{assump:randomization}). If we simply ``define'' the potential
outcomes as $\bm Y(\bm z) = \bm Y$ for all
$\bm z \in \mathcal{Z}$ so $\bm W$ consists of many identical copies
of $\bm Y$, the ``causal'' null
hypothesis $H_0:\bm  Y(\bm z) =\bm  Y(\bm z^{*}), \forall \bm z, \bm z^{*} \in
\mathcal{Z}$ would be automatically satisfied. Recall that the p-value
\eqref{eq:p-value} of a CRT is given by
\[
  P(\bm Z, \bm W) = \mathbb{P}^{*} \{T_{\bm Z}(\bm Z^{*}, \bm W)
  \leq T_{\bm Z}(\bm Z, \bm W) \mid \bm Z^{*}\in \mathcal{S}_{\bm Z},
  \bm W \},
\]
and suppose the test statistic is given by $T_{\bm z}(\bm z^{*}, \bm
W) = T(\bm z^{*}, \bm Y(\bm z^{*}))$ as in
\Cref{sec:focal-units}. Because of how the potential outcomes schedule
$\bm W$ is defined in this case, the test statistics is
equal to $T(\bm z^{*}, \bm Y)$. Furthermore, the independence of $\bm
Z$ and $\bm Y$ is equivalent to the independence of $\bm Z$ and $\bm
W$. When $\mathcal{S}_{\bm Z}$ is given by
all the permutations of $\bm Z$ as in \eqref{eq:sz-permutation}, $\bm
Z^{*} \mid \bm Z^{*} \in \mathcal{S}_{\bm Z}$ has the same
distribution as $\bm Z_{\sigma}$ where $\sigma$ is a random
permutation. Combining these observations, we see that the permutation
test of independence is identical to the conditional randomization
test of no causal effect.

In summary, the two formulations of permutation (or more broadly,
randomization) tests are unified in our framework. The CRT tests not
only a partially sharp null hypothesis about the potential outcomes
schedule $\bm W$ but also the independence of $\bm Z$ and $\bm W$
(\Cref{assump:randomization}). In the randomization model, $\bm Z
\independent \bm W$ is guaranteed by randomization, so the CRT gives a
test of the causal null hypothesis. In the population model, the causal null
hypothesis about $\bm W$ is automatically satisfied by definition, so
the CRT gives a test of independence. We would like to stress that
such a unification is only a mathematical one; the logic and
philosophy behind the two formulations are fundamentally different. In
the randomization model, inference is justified by the belief that
randomness introduced by the experimenter is exogenous. In the
population model, inference is justified by mathematical assumptions
such as exchangeability of observations. See \Cref{sec:discussion} for
further discussion.


% \qzz{}{We note that it is popular to use permutation tests for testing independence without specifying any experimenter randomness. In this case, the experimenter is usually assumed to be the nature that randomly chooses the order of $(Z_1,Y_1),\dotsc,(Z_n,Y_n)$ with equal probability in the data generating process. This means that the first two kinds of randomnesses we define in \Cref{new_intro} come from the same source. Experimenter randomnesses for testing causal null hypotheses, e.g.,  some physical acts, are clearly known by analysts. This is in contrast with assuming the random variables are i.i.d. or exchangeable, which is only a conceptualization or approximation of the reality.

% In general, if a CRT is based on an assignment distribution with an approximate or proxy density function $\hat{\pi}(\bm z)$
% instead of the true density function $\pi(\bm z)$, its type-I error guarantee is inflated as $\mathbb{P}\{P\leq \alpha\} \leq \alpha + \|\pi - \hat{\pi} \|_2$.  By viewing the standard assumptions, e.g., i.i.d. or exchangeability, as a special kind of experimenter randomness, we re-emphasize the importance of considering whether they hold or not for a practical problem.
% }

\subsection{Randomization tests for conditional independence}
\label{sec:rand-tests-cond}

Recently, there has been a growing interest in randomization tests for
conditional independence
\citep{candes2018panning,tansey2018holdout,berrett2020conditional,katsevich2020theoretical,liu2020fast}. Similar
to the last section, it is assumed that we observe independent and
identically distributed  random variables $(Z_1,Y_1,X_1),\dotsc,(Z_n,Y_n,X_n)$ and would like the
test $Z_1 \independent Y_1 \mid X_1$. This can be easily incorporated
in our framework by treating $\bm X = (X_1,\dotsc, X_n)$ as fixed; see
the last paragraph in \Cref{sec:potent-outc-fram}. In this case, the
randomization distribution of $\bm Z = (Z_1,\dotsc,Z_n)$ is given by
the conditional distribution of $\bm Z$ of $\bm X$. The same
randomization test can then be applied; see \citep[Section
4.1]{candes2018panning} for more
detail. Berrett et al.\ \cite{berrett2020conditional} extended this test by further
conditioning on the order statistics of $\bm Z$, resulting in a
permutation test.

As a remark on the terminology, the test in the last paragraph was
called ``conditional randomization test'' by
Cand{\`e}s et al.\ \cite{candes2018panning}, because the procedure conditions on $\bm
X$. However, such a conditioning is fundamentally different from
the post-experimental conditioning on $\mathcal{S}_{\bm Z}$, which we
use to distinguish conditional randomization tests from unconditional
ones. When $\bm Z$ is randomized according to $\bm X$,
conditioning on $\bm X$ is obligatory in randomization inference
because it needs to use the randomness introduced by the
experimenter (which is conditional on $\bm X$). On the other hand,
further conditioning on $\mathcal{S}_{\bm Z}$ (or on $g(\bm Z)$ as in
\Cref{prop:condition-on-function}) can be introduced by the analyst to
improve the power or make the p-value computable. For this reason, we
advocate reserving the terminology ``conditional randomization test''
for the latter case.


\subsection{Covariate imbalance and rerandomization}
\label{sec:form-part-covar}

Morgan and Rubin \cite{morgan2012rerandomization} proposed to use rerandomization to
improve covariate balance in experiments and regenerated some interest
in randomization inference
\citep{ding2015randomization,banerjee2017decision,heckman2019perry}. They
recounted a conversation
between Cochran and Fisher, in which Fisher advised to rerandomize if
some baseline covariates are not well balanced by the randomly chosen
assignment. The key insight of
Morgan and Rubin \cite{morgan2012rerandomization} is that the experiment should then
be analyzed with the rerandomization taken into account. More
specifically, rerandomization is simply a rejection sampling algorithm
for randomly choosing $\bm Z$ from
\[
  \mathcal{Z} = \{\bm z: g(\bm z) \leq \eta\},
\]
where $g(\bm z)$ measures the covariate imbalance implied by the
treatment assignment $\bm z$ and $\eta$ is the experimenter's level of
tolerance. Therefore, we simply need to use the randomization
distribution over $\mathcal{Z}$ to carry out the randomization
test. This provides an excellent example for our \emph{main thesis}
that randomization inference should be based exactly on the
randomization introduced by the experimenter and the analyst.

Another way to deal with unlucky draws of treatment assignment is to
condition on the covariate imbalance $g(\bm Z)$
\citep{hennessy2016conditional}. This inspires our
\Cref{prop:condition-on-function} in \Cref{sec:conditioning-sets}. In
our terminology, this is a conditional randomization test because the
analyst has the liberty to choose which function $g(\bm Z)$ to
condition on. On the other hand, the randomization test proposed by
Morgan and Rubin \cite{morgan2012rerandomization} is unconditional.



\subsection{Interference}
\label{sec:interference}

Much of our theoretical development in \Cref{sec:single-crt} is
inspired by an exploding literature on causal inference with
interference
\citep{hudgens2008towards,bowers2013reasoning,aronow2017estimating,athey2018exact,li2019randomization,basse2019randomization,puelz2019graph}. The
key challenge with interference is that not all potential
outcomes are imputable. This can be tackled by conditioning on a
smaller set of treatment assignments, as illustrated in
\Cref{sec:focal-units,sec:bipartite-cliques}. Many methods in this
literature
can be regarded as innovative usage of the general theory
outlined in \Cref{sec:single-crt}. In particular, null hypotheses
commonly have the level-set structure as described in
\Cref{def:level-set}, which simplifies the construction of CRT
significantly. % \textcite{basse2019randomization} appear to be the
% first who attempt to establish a general structure for a single
% CRT.

\subsection{Evidence factors for observational studies}
\label{sec:evidence-factors}

So far our discussion has been focused on randomized experiments, but
the same theory also applies to randomization inference for
observational studies \citep{rosenbaum2002observational}. Many
observational studies are analyzed under the \emph{ignorability}
or \emph{no unmeasured confounders} assumption that the treatment is
randomly assigned after conditioning
on some covariates $\bm X$. In our notation, this means that $\bm Z
\independent \bm W \mid \bm X$. However, the distribution of $\bm Z$
given $\bm X$ (often called the \emph{propensity score}) is typically
unknown and needs to be estimated \citep{rosenbaum1983central}.

Alternatively, one can match the treated units with control units to
recreate a paired or blocked randomized experiment. In the simplest
setup with a binary treatment and pair matching, each pair has one
treated unit and one control unit, but they have exactly the same
covariates. So the treatment vector
can be written as $\bm Z =(Z_{1},\dotsc,Z_{N})$ (suppose $N$ is
even) and is supported on
\[
  \mathcal{Z} = \left\{\bm z \in
    \{0,1\}^N:z_1 + z_2 = 1, \dotsc, z_{N-1} + z_{N} = 1\right\}.
\]
Typically, it is assumed that $\bm Z$ is uniformly distributed
over $\mathcal{Z}$, and a randomization test can be conducted in a
straightforward way by permuting the treatment assignments within the
pairs. The uniform distribution over $\mathcal{Z}$ can be justified by, for
example, assuming the distribution of $Z_i$ only depends on $X_i$
and are independent across $i$ \citep[Section
3.2]{rosenbaum2002observational}.\footnote{In practice, units within a pair are
not always exactly matched, which complicates the randomization
inference \citep[Section 3.6]{rosenbaum2002observational}; see also
\citep{abadie2006large} from the perspective of large sample
properties of the matching estimator of average treatment
effect. Another complication being omitted here is that the matched sets are
typically constructed from a larger set of units. The
standard permutation test can be regarded as a CRT that conditions on
$\mathcal{Z}$. However, our general theory in \Cref{sec:single-crt}
may be inapplicable because $\mathcal{Z}$ depends on treatment
variables of a larger set of units and may not induce a partition. To our
knowledge, this subtle issue has not been acknowledged in the
literature yet.}

When there are concerns about unmeasured confounders,
Rosenbaum \cite{rosenbaum1987sensitivity,rosenbaum2002observational}
introduces a general sensitivity analysis framework of the
ignorability assumption. In essence, Rosenbaum's sensitivity model
allows the distribution $\bm Z$ to be non-uniform over $\mathcal{Z}$,
but the ``degree'' of non-uniformness is bounded. More specifically,
it assumes that
\begin{equation}
  \label{eq:rosenbaum-model}
  \frac{1}{1 + \Gamma} \leq \mathbb{P}(Z_i = 1) \leq \frac{\Gamma}{1 +
    \Gamma},~i = 1,\dotsc,N,
\end{equation}
where $\Gamma \geq 1$ is chosen by the analyst.

Let $\Pi$ be the set of distributions of $\bm Z$ that satisfy
\eqref{eq:rosenbaum-model}. We denote the p-value in
\eqref{eq:p-value} as $P(\bm Z, \bm Y; \pi)$ to emphasize that it
depends on the unknown randomization distribution $\pi$ of
$\bm Z$. For simplicity, we will assume that the p-value
is always computable when discussing sensitivity analysis. Because
each p-value $P(\bm Z, \bm Y; \pi)$ satisfies
\eqref{eq:stoc-domi-marginal} under the null hypothesis if $\pi$ is
indeed the distribution of $\bm Z$, by applying the union bound,
\begin{equation}
  \label{eq:sensitivity-p-value}
  P(\bm Z, \bm Y) = \sup_{\pi \in \Pi} P(\bm Z, \bm Y; \pi)
\end{equation}
satisfies \eqref{eq:stoc-domi-marginal} (stochastically dominates the
uniform distribution over $[0,1]$) if the actual distribution of $\bm
Z$ is indeed in
$\Pi$. Rosenbaum \cite{rosenbaum1987sensitivity,rosenbaum2002observational}
provides analytical solutions to the optimization problem in
\eqref{eq:sensitivity-p-value} for a class of sign-score statistics.

In subsequent works, Rosenbaum
\cite{rosenbaum2010evidence,rosenbaum2011some,rosenbaum2017general}
introduces a concept for observational
studies called ``evidence factors''. This is closely related to our
theory of multiple CRTs in
\Cref{sec:multiple-crt}. Loosely speaking, a causal theory can usually
be represented by several hypotheses. For example, the conclusion
``smoking does not cause lung cancer'' entails at least two
hypotheses: whether or not a person smokes does not alter the risk of
lung cancer, and given that the person smokes, the amount of
cigarettes he or she smokes does not alter the risk of lung cancer
either. Therefore, we can then reject null causal theory if either
hypothesis is rejected. When there are concerns about unmeasured
confounders, we may represent the evidence factors by the p-values
obtained from suitable sensitivity analyses. This typically requires
us to specify a sensitivity model $\Pi$ for each hypothesis and
computing the upper bound in \eqref{eq:sensitivity-p-value}.

Rosenbaum's key observation is that in certain problems, these
evidence factors (p-value upper bounds) are ``independent'' in the sense that they satisfy \eqref{equ:dominance-3} when all the null
hypotheses are true. This allows one to test the global null
and the partial conjunction hypotheses using standard methods
\citep{karmakar2019integrating}. Rosenbaum \cite{rosenbaum2010evidence,rosenbaum2011some}
provides some concrete examples of evidence factors, which essentially
correspond to the sequential CRTs described in \Cref{sec:sequential-crts}.

Rosenbaum \cite{rosenbaum2017general} demonstrates that the permutation
groups of a general class of ``independent'' evidence factors have a
knit product structure. Similar to our remark on Southworth et al.\
\cite{southworth2009properties}
in \Cref{sec:permutation-tests}, we believe that the requirement that
$\mathcal{Z}$ is a group or has a knit product structure is not
necessary. Instead, the key is to construct sequential CRTs that
satisfy the conditions in \Cref{prop:nested}. Because the conditions
in \Cref{prop:nested} do not rely on the distribution of $\bm Z$,
the key stochastic dominance result \eqref{equ:dominance-3} holds for
the p-values $P^{(1)}(\bm Z, \bm Y; \pi), \dotsc, P^{(K)}(\bm Z, \bm
Y; \pi)$ for any distribution $\pi$ of $\bm Z$. By computing the
p-value suprema as in \eqref{eq:sensitivity-p-value}, we see that the
evidence factors satisfy the same stochastic dominance result if the sensitivity model is correct.

\subsection{Conformal prediction}
\label{sec:conformal-prediction}

Conformal prediction is another topic related to randomization
inference that is receiving growing interest in statistics and machine learning
\citep{vovk2005algorithmic,shafer2008tutorial,lei13distribution,lei18distribution}. Consider
a typical regression problem where the data points
$(X_1,Y_1),\dotsc,(X_{N},Y_{N})$ are drawn exchangeably from the same
distribution and $Y_N$ is unobserved. We would like to construct a
prediction interval $\hat{\mathcal{C}}(X_N)$ for the next observation
$(X_N,Y_N)$ such that
\[
  \mathbb{P}(Y_N \in \hat{\mathcal{C}}(X_N)) \leq 1 - \alpha.
\]
The key idea of conformal inference is that the exchangeability of
$(X_1,Y_1),\dotsc, (X_N,Y_N)$ allows us to
test the null hypothesis $H_0:Y_N = y$ using permutation tests. More
concretely, we may fit \emph{any} regression model to
$(X_1,Y_1),\dotsc,(X_{N-1},Y_{N-1}),(X_N,y)$ and let the p-value be
one minus the percentile of the absolute residual of $(X_N,y)$ among
all $N$ absolute regression residuals. Intuitively, a large
residual of $(X_N,y)$ indicates that the prediction $(X_N,y)$
``conforms'' poorly with the other observations, so $H_0:Y_N = y$ should be
rejected.

We argue that conformal prediction is a special instance of
the randomization inference described in \Cref{sec:single-crt}. The
key idea is to view random sampling as a
kind of randomization. Notice that conformal prediction implicitly
conditions on the unordered data points $(X_1,Y_1),\dotsc,(X_N,Y_N)$. To
make this more explicit, let the treatment variable $Z$ be the
order of the observations, which is a random permutation of $[N]$ or
equivalently a random bijection from $[N]$ to $[N]$. The
``potential outcomes'' are given by
\begin{equation}
  \label{eq:conformal-counterfactual}
  \bm Y(z)  = \left( (X_{z(1)},Y_{z(1)}),\dotsc,(X_{z(N)},Y_{z(N)}) \right),
%  \begin{cases}
%    (X_{z(i)}, Y_{z(i)}), & \text{if}~i=1,\dotsc,N-1, \\
%    X_{z(N)}, & \text{if}~i=N,
%  \end{cases}
\end{equation}
where $Y_{z(N)}$ is unobserved (that is, the observed $\bm Y$ is the
first $2N-1$ elements of $\bm Y(\bm Z)$). The notation $\bm Y$ is
overloaded here to be consistent with \Cref{sec:single-crt}. The
``potential outcomes schedule'' in our setup is
$\bm W = \left\{\bm Y(z) : \text{ $z$ is a permutation of $[N]$}\right\}$.

The null hypothesis in conformal prediction can be represented
as a regression model $f(x)$ such that the missing $Y_{z(N)}$ is imputed by
$f(X_{z(N)})$. This is a sharp null hypothesis and our theory in
\Cref{sec:single-crt} can be directly used to construct a
randomization test. Notice that the key randomization assumption $Z
\independent \bm W$ in our theory (\Cref{assump:randomization}) is
justified here by the assumption that $(X_1,Y_1),\dotsc,(X_N,Y_N)$ are
exchangeable. In other words, we may view random sampling as a form of
randomizing the order of the observations.

The above argument can be extended to allow ``covariate shift'' in the
next observation $X_N$
\citep{tibshirani2019conformal,hu20distribution}. The key idea is,
again, to consider the randomization involved in sampling. For this we need
to consider a (potentially infinite) super-population $(X_i,Y_i)_{i
  \in \mathcal{I}}$. The ``treatment'' $Z: [N] \to \mathcal{I}$
selects which units are observed. For example, $Z(1) = i$ means that
$(X_i,Y_i)$ is the first data point. The ``potential outcomes'' are still
given by \eqref{eq:conformal-counterfactual}. By conditioning on
unordered $Z$, we can obtain a conditional randomization test
for the unobserved $Y_{z(N)}$. Covariate shift in $X_N$ can be easily
incorporated by conditioning on $(X_{Z(1)},\dotsc, X_{Z(N)})$ and deriving the
conditional distribution of $Z$. For
example, suppose the first $N-1$ units
are sampled from the population according to a covariate distribution
$\pi_1(\bm x)$ and the last unit is sampled according to another
covariate distribution $\pi_2(\bm x)$, that is,
\begin{equation}
  \label{eq:cov-shift-dist}
  \begin{split}
  &\mathbb{P}(Z(k) = i) \propto \pi_1(X_i)~\text{for}~k=1,\dotsc,N-1,i \in
  \mathcal{I}, \\
  &\mathbb{P}(Z(N) = i) \propto \pi_2(X_i)~\text{for}~i \in
  \mathcal{I}.
  \end{split}
\end{equation}
For simplicity, we assume the data points are sampled without
replacement. Then the unordered $Z= \{Z(1),\dotsc,Z(N)\}$ is a set
$\mathcal{S} = \{s_1,\dotsc,s_N\}$ of $N$ distinct units. Let $\bm X =
(X_{s_1},\dotsc,X_{s_N})$. The conditional randomization
distribution of $Z$ is given by
\begin{align*}
  \P\left(Z(N) = s_i \mid \bm X, \mathcal{S}\right)
  % &
    \propto % \sum_{z:z(N)=s_i }
      \pi_2(X_{z(N)})  \prod_{j =1}^{N-1}\pi_1(X_{z(j)})         % \\
 % &= \frac{\pi_2(X_{s_i})q(Y_{s_i}\mid X_{s_i})}{\pi_1(X_{s_i})q(Y_{s_i}\mid X_{s_i})}\sum_{z:z(N)=s_i } \prod_{j =1}^{N}\pi_1(X_{z(j)})q(Y_{z(j)}\mid X_{z(j)})\\
 % &
   \propto \frac{\pi_2(X_{s_i})}{\pi_1(X_{s_i})},~i=1,\dotsc,N,
\end{align*}
by using the fact that the product $\prod_{j=1}^{N}\pi_1(X_{z(j)}) =
\prod_{j=1}^N$ $\pi_1(X_{s_j})$ only depends on $\mathcal{S}$.
By normalizing the probabilities, we obtain
\[
  \P\left(Z(N) = s_i \mid \bm X,\mathcal{S}\right)
  =
  \frac{\pi_2(X_{s_i})/\pi_1(X_{s_i})}{\sum_{j=1}^N\pi_2(X_{s_j})/\pi_1(X_{s_j})},~ i=1,\dotsc,N.
\]
% The same result holds if one further includes a common term $q(Y_i
% \mid X_i)$ ($q(Y \mid X)$ can be any conditional density function of $Y$ given $X$) in the
% randomization distributions \eqref{eq:cov-shift-dist} and conditions
% on the data points $(X_{s_1},Y_{s_1}),\dotsc, (X_{s_N},Y_{s_N})$, as the common term $\prod_{j=1}^N
% q(Y_{s_j}\mid X_{s_j})$ is cancelled during normalization.

The last display equation was termed ``weighted exchangeability'' in
\cite{tibshirani2019conformal}. Again, we would like to stress
that exchangeability (unweighted or weighted) is not necessary
here. What is necessary is a careful consideration of the
randomization $\bm Z$ in the problem. This could be
either explicit as in a physical intervention, or implicit as in
random sampling. Once the randomization distribution of $\bm Z$ is
given and a suitable conditioning set $\mathcal{S}_{\bm Z}$ is found,
the rest is just a straightforward application of the general
conditional randomization test. For example, sampling schemes that are
more general than \eqref{eq:cov-shift-dist} can in principle be
allowed, although the conditional randomization distribution might not
be as simple as above.




==> Figures/0_Abstract.tex <==
We establish a general sufficient condition for
constructing multiple ``nearly independent'' conditional randomization
tests, in the sense that the joint distribution of their p-values is
almost uniform under the global null. This property implies that the
tests are jointly valid and can be combined using standard
methods. Our theory generalizes existing techniques in the literature
that use independent treatments, sequential treatments, or
post-randomization, to construct multiple randomization tests. In
particular, it places no condition on the experimental design,
allowing for arbitrary treatment variables, assignment mechanisms and
unit interference. The flexibility of this framework is illustrated through
developing conditional randomization tests for lagged treatment
effects in stepped-wedge randomized controlled trials. 
We compare the efficiency and robustness of the popular mixed-effect models and the proposed conditional randomization
tests using simulated experiments and real trial data.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Figures/1_Introduction.tex <==



\section{Introduction}\label{new_intro}

Randomized experiments over time or space have produced increasingly more opportunities to apply randomization tests in social and biomedical sciences. These tests are purely based on the physical act of randomization. They can provide finite-sample valid p-values and confidence intervals for inference with no distributional assumption whatsoever. This unique property makes them appealing to practitioners, considering that any other inference methods are more or less sensitive to model misspecification. 

However, many  causal questions arising from complex experiments can not be simply addressed by running a simple randomization test. Exploring the role of conditioning has been the recent focus of the literature. Some notable advances include {\it conditional randomization tests} (CRTs) for meta-analysis \citep{zheng2008multi}, covariate adjustment \citep{hennessy2016conditional}, and unit interference
\citep{athey2018exact,basse2019randomization,puelz2019graph}. In these tests, conditioning is the key to test causal hypotheses that are more precise. For example, suppose that in an experiment, units (i.e. individuals) are gradually randomized  to receive a treatment over time, and we want to know if the treatment is effective right after it is assigned. A conditional randomization test can compare the units who are treated shortly and never treated. The inference is based on an artificial experiment only involving units that are relevant to our hypothesis. The test is valid if the conditioning event is chosen properly. More theory and background of a single CRT can be found in  \Cref{sec:single-crt} and our accompanying article \citep{zhangzhao2022}. In this article, we take a step forward to explore the following two applications that call for multiple CRTs.

\begin{example}[Lagged treatment effect in stepped-wedge trials \citep{hussey2007design}]\label{label:s_exp}
The stepped-wedge randomized controlled trial is a monotonic cross-over design in which all units start out in the control and then
cross over to the treatment randomly at staggered times. This design is also known as \emph{staggered adoption} \citep{abraham2018estimating,athey2018design} in econometrics. It is now widely used  in medical and policy research, especially in applications that (1) can not randomize the treatment to every unit at once, or (2) want every unit to eventually receive the treatment that is seemingly effective.

Comparing outcomes over time is a natural way to estimate lagged effects in stepped-wedge designs. Mixed-effects models can be easily applied for this purpose \citep{hussey2007design,hemming2018reporting,li2021mixed}. But they are unreliable for inference (e.g. have inflated type I error and poor confidence coverage) when the model is misspecified
\citep{thompson2017bias,ji2017randomization}. In light of this, randomization tests have been proposed to test the
global null hypothesis of no treatment effect (i.e. zero effect at any time lag)
\citep{ji2017randomization,wang2017use,thompson2018robust,hughes2020rob}. However, testing the global null is inadequate to address some common questions in applied research such as if the effect is immediate or delayed, and if the effect is short-term or long-term. In \Cref{sec:swd}, we fill this gap by proposing a solution based on multiple CRTs. Each CRT is based on an artificial experiment that randomly starts the treatment for the untreated units at a particular time step, then it tests the effect on their outcomes after the time lag of interest. Repeat this process at different time steps give rise to multiple CRTs. We keep these CRTs jointly valid by choosing their conditioning events carefully. We can combine them to test the same lagged effect recurring over time. We will compare our method with mixed-effects models on two real stepped-wedge trials from \citet{twiskanalysis2021}.

\end{example}

\begin{example}[Testing the range of spillover effect under general interference]\label{label:c_exp}
In a randomized experiment over a space or network, it is reasonable to believe that the neighbouring units can interfere with each other. The treatment assigned to a particular unit may have a spillover effect on its neighbours.
For example, \citet{jayachandran2017cash}  conducted a randomized controlled trial to study if payments for ecosystem services can reduce deforestation in Uganda.
After receiving the payments, the forest owners shall conserve more forests in their villages. However, there maybe a spillover effect---they deforest more in the nearby untreated villages.   
% For example, \citet{collazos2021hot} conducted a large-scale randomized experiment to study if increasing daily police presence in some fixed streets can reduce the crime rate in Medell\'{i}n, Colombia. Their result suggests that %the crime rate also decreases significantly in the areas close to those treated streets. 
 CRTs for spillover effects are developed recently by \citet{aronow2012general,athey2018exact,basse2019randomization,puelz2019graph}. A single CRT can only test if the spillover effect exists within a chosen distance.  Assessing how far the effect can spillover is important for many applications that consider policy optimization, e.g., maximizing the forest conservation by assigning the payments to a few villages.
If we run multiple CRTs for different distances,  the results from different tests are dependent so interpret them together will lose the type I error control granted by the physical act of randomization. In \Cref{sec:spillover}, we propose a method to construct multiple independent CRTs for the spillover effect at different distances. Intuitively, the units' locations in the space determine if they are suitable for testing the spillover effect at short or long distances. Our CRTs follow from a sequence of artificial experiments designed according to the units' locations. The designs allow the effect to spread at different distances in the space. The tests can be combined to detect how quick the spillover effect vanishes as the distance increases. We will demonstrate this method using the forest trial data \citep{jayachandran2017cash}.

\end{example}
%The rest of this article is organized as follows.  In \Cref{sec:single-crt}, we provide a brief review of a single CRT and then  introduce the theoretical results that support our multiple CRTs methods used in the applications introduced above (\Cref{sec:swd,sec:spillover}). The main result is a sufficient condition under which the p-values of multiple CRTs can be jointly valid, meaning that their joint distribution is nearly uniform. In such cases, the tests can be combined by standard methods such as Fisher's method and can be
%easily extended to simultaneous testing using the closed testing procedure
%\citep{marcus1976closed}. We base our condition solely  on the conditioning events and test statistics of the CRTs. We place no restriction on the type of treatment variable, assignment mechanism and unit interference.
%In  \Cref{sec:experiment},  we further validate our methods through a set of simulations. 
%\Cref{sec:discussion} concludes the article with some discussion on potential avenues for future research.



==> Figures/2_Single_CRT.tex <==

\section{Review: A single conditional randomization test}
\label{sec:single-crt}

% This section provides some background on conditional randomization
% tests; A more thorough review can be found in an accompanying article
% by the authors.

% \subsection{A single CRT}

We start with a brief review of conditional randomization tests; see
\citet{zhangzhao2022} for more details and discussion.

Consider an arbitrary randomized experiment on $N$ units. Let $\bm Z
$ denote the treatment assignment that is randomized in
the experiment which takes value in $\mathcal{Z}$.
For every unit $i\in [N]:=\{1,\cdots,N \},$ we denote all its \emph{potential outcomes} by $(Y_i(\bm z)\mid \bm z\in \mathcal{Z})$. Let  $\bm Y(\bm z) = (Y_1(\bm z), \dotsc, Y_N(\bm z)).$ After $\bm Z$ is randomized, we observe one outcome $Y_i$ for every
unit $i$.  We assume all the observed outcomes $\bm Y =
(Y_1,\dotsc,Y_N)$ are consistent in the sense that $\bm Y = \bm Y(\bm
Z).$

The \emph{potential outcomes schedule} for all units and treatment
assignments is denoted by $\bm W = (\bm Y (\bm z): \bm z \in
\mathcal{Z}) \in \mathcal{W}$. Treatment effect (e.g. the lagged effect and spillover
effect discussed above) is defined as the contrast between some
potential outcomes in $\bm W$. By randomizing $\bm Z$, the experiment
establishes independence between $\bm Z$ and $\bm W$ that
eliminates all confounding factors between the treatment and the
outcome. This is stated as a formal assumption below.

\begin{assumption}[Randomized experiment] \label{assump:randomization}
  $\bm Z \independent \bm W$ and the density function $\pi(\cdot)$ of
  $\bm Z$  is known and positive everywhere.
\end{assumption}


% Independence between $\bm Z$ and $\bm W$ is justified by the
% randomization. We may view $\bm Z$ and $\bm W$ as defined on two
% separate probability spaces as $\bm W$ represents randomness in
% nature and consider the product probability space. If
% $\bm Z$ is randomized according to some $\bm X$ (possibly some
% observed attributes of the units), we may assume that $\bm Z
% \independent \bm W \mid \bm X$. To simplify the exposition, we will
% simply treat $\bm X$ as fixed, so $\bm Z \independent \bm W$ is true
% in the conditional probability space given $\bm X$.

We are interested in testing sharp
causal hypotheses about the treatment effect that allow us to impute
some entries of $\bm W$ from $\bm Y$. The simplest example is the
global null
hypothesis that says $\bm Y(\bm z) = \bm Y(\bm z')$ for all $\bm z,
\bm z' \in \mathcal{Z}$. Under such a fully sharp hypothesis, all
potential outcomes in  $\bm W$ can be imputed using the observed
outcome $\bm Y$.
However, we are often interested in testing more granular hypotheses
that only allow us to impute part of $\bm W$. In this case,
conditioning is useful tool to exclude non-imputable potential
outcomes. Specifically, a conditional randomization test is defined
as follows.

\begin{definition}\label{def:CRT}
  A \emph{conditional randomization test} (CRT) for the treatment  $\bm Z$ is defined by
  % \begin{enumerate}
  % \item\label{item:crt_1} A
  a countable \emph{partition} $\mathcal{R} =
  \{\mathcal{S}_m\}_{m=1}^{\infty}$ of $\mathcal{Z}$ and
  a collection of \emph{test statistics}
  $\{T_m(\cdot,\cdot) \}_{m=1}^{\infty} $, where
  $T_m:\mathcal{Z} \times \mathcal{W} \to \mathbb{R}$ is a
  (measurable) function. With an abuse of notation, let
  $\mathcal{S}_{\bm z}$ be the set in the partition $\mathcal{R}$
  that contains $\bm z$, and let $T_{\bm z}$ be the
  corresponding test statistic. The \emph{p-value} of the CRT is then
  given by
  \begin{equation}
    \label{eq:p-value}
    P(\bm Z, \bm W) = \mathbb{P}^{*} \{T_{\bm Z}(\bm Z^{*}, \bm W)
    \leq T_{\bm Z}(\bm Z, \bm W) \mid \bm Z^{*}\in \mathcal{S}_{\bm
      Z}, \bm Z, \bm W \},
  \end{equation}
  where $\bm Z^{*}$ is an independent copy of $\bm Z$ conditional on
  $\bm W$, and the notation $\mathbb{P}^{*}$ is used to emphasize that
  the probability is taken only over the randomness of $\bm Z^{*}$.
\end{definition}

In words, the CRT compares the test statistic at the observed
treatment $\bm Z$ with all other potential treatment assignments $\bm
Z^{*}$ that are in the same equivalence class as $\bm Z$. One might
think of $\mathcal{S}_{\bm Z}$ as the ``orbit'' of $\bm Z$, although
$\mathcal{S}_{\bm Z}$ does not need to be the orbit of a group action
\citep[sec.\ 15.2]{lehmann2006testing}.

Note that this definition of a CRT does not refer to a null
hypothesis, and the p-value is a function of the potential outcomes
schedule $\bm W$ instead of the observed outcomes $\bm Y$. A benefit
of this representation is that the CRT is always a valid test, as
indicated by the next result, and the role of the null hypothesis is
to impute the potential outcomes so that the p-value is
computable. See \citet{zhangzhao2022} for further discussion.

Let $\mathcal{G} = \sigma\left( \mathcal{S}_{\bm Z}
\right)$ denote the $\sigma$-algebra generated by the conditioning
event $\mathcal{S}_{\bm Z}$.

% Recall that an unconditional randomization test is implemented by
% comparing the test statistics under the realized $\bm Z$ and all the
% assignments $\bm z^{*}\in \mathcal{Z}$.
% Here we let $\mathcal{S}_{\bm z}$ denote the conditioning set used in the CRT when $\bm Z=\bm z.$
% For any $\bm z \in \mathcal{S}_m$, we write $\mathcal{S}_{\bm z} = \mathcal{S}_m$ and $T_{\bm z}(\cdot,\cdot) = T_m(\cdot,\cdot)$. In other words,  $\mathcal{S}_m$ is the conditioning set used in the CRT whenever $\bm Z=\bm z\in S_m.$
% The p-value \eqref{eq:p-value} is obtained by only comparing the the test statistics under $\bm Z$ and all the assignments $\bm z^{*}\in S_{\bm Z}$.
% Finally, if the $\mathcal{S}_{\bm z} =\mathcal{Z}$ for all $\bm z,$ i.e., the partition is a trivial singleton, the CRT reduces to an unconditional randomization test.

% Under \Cref{assump:randomization}, by the proof of unconditional randomization tests, it is straightforward to  that
% $ \P\left\{ P(\bm Z, \bm W) \leq \alpha \mid \bm Z\in \mathcal{S}_m, \bm W\right\} \leq \alpha, \forall \alpha\in[0,1] \text{ and } m.$
% Then the p-value is also valid conditioning on any countable unions of the sets in $\mathcal R = \{\mathcal{S}_m\}.$
% The collection of all possible unions of the sets in $\mathcal R$ is the generated $\sigma$-algebra  $\mathcal{G} = \sigma\left( \mathcal R \right).$
% Overall, the validity of a single CRT is formalized as follows.

\begin{theorem}\label{thm:valid}
  Under \Cref{assump:randomization},  the p-value in
  \eqref{eq:p-value} satisfies that, for any $\alpha \in [0,1],$
  \begin{equation}
    \label{eq:stoc-domi-sigma}
    \P\left\{ P(\bm Z, \bm W) \leq \alpha \mid \mathcal{G}, \bm W\right\} = \sum_{m} 1_{\{\bm Z \in \mathcal{S}_m\}} \P\left\{ P(\bm Z, \bm W) \leq \alpha \mid
      \bm Z \in \mathcal{S}_m, \bm W\right\}
    \leq \alpha,
  \end{equation}
  In consequence, the CRT is valid in the sense that  $\mathbb{P}\left\{
    P(\bm Z, \bm W)\leq \alpha\right\}\leq \alpha, \forall
  \alpha\in[0,1].$
\end{theorem}

The proof of \Cref{thm:valid} can be found in \citet{zhangzhao2022}.
By further randomizing the rejection, the inequality
\eqref{eq:stoc-domi-sigma} can be replaced with an equality for all
$\alpha \in [0,1]$; see \citet[Equation
5.51]{lehmann2006testing}. For this reason, we shall refer to the
CRT as ``nearly'' exact and the multiple CRTs introduced below as
``nearly'' independent.

\section{Sequential conditional randomization tests}
\label{sec:sequential-crts}

Our main goal is to characterize when multiple CRTs, as defined by
the partitions
$\mathcal{R}^{(k)} = \big\{\mathcal{S}^{(k)}_m\big\}_{m=1}^{\infty}$
and test statistics $\big\{T_m^{(k)} \big\}_{m=1}^{\infty}$ for $k =
1,\dots,K$, are ``nearly''
independent. By this we mean the corresponding p-values
$P^{(1)}(\bm Z, \bm W), \dotsc, P^{(K)}(\bm Z, \bm W)$ satisfy
\begin{equation}\label{equ:dominance-3}
  \mathbb{P}\left\{P^{(1)}(\bm Z, \bm W) \leq \alpha^{(1)},\dotsc, P^{(K)}(\bm
    Z, \bm W) \leq \alpha^{(K)}\right\}\leq
  \prod_{k=1}^{K}\alpha^{(k)},~\forall \alpha^{(1)},\dots,\alpha^{(K)} \in [0,1].
\end{equation}
In this section we are concerned with a sequential construction of
CRTs that satisfy \eqref{equ:dominance-3}. A more general theory is
described in \Cref{sec:multiple-crt}.

We write $ \mathcal{S}_{\bm z}^{(k)} =  \mathcal{S}_m^{(k)}$ for all
$\bm z\in \mathcal{S}_m^{(k)}$. % We assume each $P^{(k)}(\bm Z, \bm W)$
% satisfies \eqref{eq:stoc-domi-sigma}, i.e.,
% \begin{equation}
%   \label{eq:stoc-domi}
%   \mathbb{P}\left\{ P^{(k)}(\bm Z, \bm W)\leq \alpha \mid \bm Z \in
%     \mathcal{S}_{\bm z}^{(k)}, \bm
%     W\right\}\leq \alpha, \quad \forall \alpha\in[0,1]  \text{ and } \bm z \in
%   \mathcal{Z}.
% \end{equation}
% Fix $m$ and $k\neq k'$,  $\mathcal{S}_m^{(k)}$ and $\mathcal{S}_m^{(k')}$  may be irrelevant to each other.
This notation allows us to discuss overlapping conditioning sets from
different CRTs. Consider the following result. % We call the CRTs sequential if their conditioning sets
% are nested as in the proposition below.
\begin{theorem} \label{prop:nested}
  Under  \Cref{assump:randomization}, equation \eqref{equ:dominance-3} holds if
  \begin{enumerate}
  \item\label{item:6_1} $\mathcal{S}_{\bm z}^{(1)} \supseteq \dotsb \supseteq
    \mathcal{S}_{\bm z}^{(K)}$ for all $\bm z \in \mathcal{Z}$; and
  \item\label{item:6_2} $T_{\bm z}^{(j)}(\bm z,
    \bm W)$ does not depends on $\bm z$ when $\bm z$ is restricted to
    $\bm z \in \mathcal{S}_m^{(k)}$ for any $m$ and $1 \leq j<k \leq K$;
  \end{enumerate}
\end{theorem}

In words, this result says that if each CRT conditions on the
information used in the previous CRTs, then the CRTs are nearly
independent. To see this, let $\mathcal{G}^{(k)} =
\sigma(\mathcal{S}_{\bm Z}^{(k)})$ denote the $\sigma$-algebra
generated by the conditioning event in test $k$. The two conditions in
\Cref{prop:nested} then imply that
\[
  \mathcal{G}^{(j)} \subseteq \mathcal{G}^{(k)} \quad
  \text{and} \quad T_{\bm Z}^{(j)}(\bm Z, \bm W) \independent
    \bm Z \mid \mathcal{G}^{(k)},~\forall 1 \leq j < k \leq K.
\]
% their generated $\sigma$-algebras satisfy that
% they use a nested sequence of partitions
% so that $\mathcal{S}_{\bm z}^{(1)}
% \supseteq \dotsb \supseteq \mathcal{S}_{\bm z}^{(K)}$ for all $\bm z$.

Next, we prove \Cref{prop:nested} when $K = 2$. Let $\psi^{(k)}(\bm Z, \bm
W) = 1_{\{P^{(k)}(\bm Z, \bm W) \leq \alpha^{(k)}\}}$,
$k=1,\dots,K$. For any $\bm w \in \mathcal{W}$, the conditions above imply that $\psi^{(1)}(\bm Z, \bm
w)$ is $\mathcal{G}^{(2)}$-measurable. By the law of iterated expectation,
\begin{align*}
  &  \mathbb{P}\left\{P^{(1)}(\bm Z, \bm w) \leq \alpha^{(1)}, P^{(2)}(\bm Z,
    \bm w) \leq \alpha^{(2)} \mid \mathcal{G}^{(1)}\right\} \\
  =\ &  \mathbb{E}\left\{\psi^{(1)}(\bm Z, \bm w) \psi^{(2)}(\bm Z, \bm w) \mid
    \mathcal{G}^{(1)}\right\} \\
  =\ &  \mathbb{E}\left\{\mathbb{E}\left[\psi^{(1)}(\bm Z, \bm w) \psi^{(2)}(\bm Z, \bm w) \mid
       \mathcal{G}^{(2)}\right] \mid \mathcal{G}^{(1)}\right\} \\
  =\ & \mathbb{E}\left\{\psi^{(1)}(\bm Z, \bm w) \mathbb{E}\left[\psi^{(2)}(\bm Z, \bm w) \mid
       \mathcal{G}^{(2)}\right] \mid \mathcal{G}^{(1)}\right\} \\
  \leq \ &  \alpha^{(2)} \mathbb{E}\left\{\psi^{(1)}(\bm Z, \bm w) \mid
           \mathcal{G}^{(1)}\right\} \\
  \leq \ &  \alpha^{(1)} \alpha^{(2)}.
\end{align*}
This proof can be easily generalized to $K > 2$ tests. Taking
expectation over $\mathcal{G}^{(1)} $ gives
\eqref{equ:dominance-3}.

It is easy to see that the above proof still goes through if the
conditional independence $\psi^{(1)}(\bm Z, \bm
w) \independent \psi^{(2)}(\bm Z, \bm w) \mid \mathcal{G}^{(2)}$ holds
(which is of course implied by the assumption that $\psi^{(1)}(\bm Z,
\bm w)$ is $\mathcal{G}^{(2)}$-measurable). In \Cref{sec:multiple-crt}
we state a more general theorem that does not require the CRTs to be
nested in the sense above.

\Cref{prop:nested} motivates the following general construction of
sequential CRTs. Suppose the treatment $\bm z$ can be separated into
$K$ components: $\bm z = (\bm z^{(1)},\dots,\bm z^{(K)}) \in
\mathcal{Z}^{(1)} \times \dots \times \mathcal{Z}^{(K)}$. We may then
construct a sequence of $K$ CRTs, in which the $k$th CRT conditions on
$\bm Z^{(1)},\dots,\bm Z^{(k-1)}$ and uses the randomization
distribution of $\bm Z^{(k)}$ to test a null hypothesis. Formally, for
any
subset $\mathcal{J}$ of $[K]$, let $\bm z^{\mathcal{J}}$ denote $(\bm
z^{(k)})_{k \in \mathcal{J}}$, so $\bm z^{[k]} = (\bm z^{(1)},\dots,
\bm z^{(k)})$. Let the $k$th CRT be defined by the conditioning set
(we use the convention $[0] = \emptyset$)
\[
  \mathcal{S}^{(k)}_{\bm z} = \left\{\bm z^{*} = (\bm z^{*(1)},\dots,\bm
  z^{*(K)}): \bm z^{*[k-1]} = \bm z^{[k-1]}\right\}
\]
and the test statistic $T^{(k)}: \mathcal{Z}^{[k]} \times \mathcal{W}
\to \mathbb{R}$ be a function of $\bm z^{[k]}$ and $\bm W$. It is easy
to see that $\mathcal{G}^{(k)} = \sigma(\mathcal{S}_{\bm Z}^{(k)}) =
\sigma(\bm Z^{[k-1]})$, and both conditions in \Cref{prop:nested} are
satisfied.

In the next three sections, we illustrate the application of
sequential conditional randomization tests in three examples: (1)
evidence factors for observational studies; (2) lagged treatment
effect in stepped-wedge trials; (3) spillover effect in randomized
trials with interference.

\section{Application 1: Evidence factors}
\label{sec:evid-fact-observ}

% Our theory assumes a randomized experiment, and it is interesting to
% study if the same theory also applies to randomization inference for
% observational studies. Matching by observed confounders is often used
% to mimic an randomized experiment using
% observational study. The complication here is that the matched sets
% are often a random subset of units that depend on the treatment
% assignment, so our theory cannot directly apply because it assumes
% $\mathcal{Z}$ is fixed. This subtle issue is usually ignored
% in the randomization inference literature, which typically treats
% the matched observational sample as a block-randomized experiment
% \citep{rosenbaum2002observational}.

\citet{rosenbaum2010evidence,rosenbaum2017general}
developed a concept called ``evidence factors'' for observational
studies, which are essentially pieces of evidence different regarding
different aspects of an abstract causal hypothesis. Roughly speaking,
each evidence factor is characterized by an p-value upper bound
obtained from a sensitivity analyses for a different (partially) sharp
null hypothesis. Rosenbaum's key observation is that in certain
problems, these evidence factors are nearly independent in the sense
that the p-value upper bounds satisfy \eqref{equ:dominance-3}.

Next, we shall use the theory of sequential CRTs in
\Cref{sec:sequential-crts} to explain why certain evidence factors are
nearly independent. Consider the example in
\citet{rosenbaum2017general} that concerns the causal effect of
smoking on periodontal disease. Each subject in this analysis
is categorized as a ``non-smoker'', ``light smoker'', or ``heavy
smoker''. The main idea of \citet{rosenbaum2017general} is to
represent the exposure as two indicators, one for smoking and one for
heavy smoking. That is, let the exposure be $\bm Z = (\bm Z^{(1)},
\bm Z^{(2)})$, where $\bm Z^{(1)}$ and $\bm Z^{(2)}$ are
$N$-dimensional binary variables, $Z^{(1)}_i = 1$ (0) means subject $i$ is
a smoker (not a smoker), and $Z^{(2)}_i = 1$ (0) means subject $i$ is a
heavy smoker (not a heavy smoker). Rosenbaum then constructed a
randomization test by comparing the outcomes of the smokers with the
non-smokers, and another randomization test by comparing the outcomes
of the heavy smokers with the light smokers. Thus, the first test
statistic is a function of $\bm Z^{(1)}$, the second test
statistic is a function of $\bm Z^{(2)}$, and the second test
conditions on $\bm Z^{(1)}$. This is exactly the structure of
sequential CRTs described in \Cref{sec:sequential-crts}.

As the dataset analyzed by \citet{rosenbaum2017general} is
observational, the smoking exposure $\bm Z$ is not
randomized. Rosenbaum constructed pairs of smoker and non-smoker
that are matched for age, gender, education, income, and ethnicity. He
then constructed independent sensitivity analyses using the two
randomization tests. We will not dive deeply into the sensitivity
models used by \citet{rosenbaum2017general}; rather we will let
$\Pi^{(k)}$ denote the collection of all distributions $\pi^{(k)}$ of
$\bm Z^{(k)}$ that are allowed by the sensitivity model,
$k=1,2$. Rosenbaum obtained closed form expressions of the upper
bounding p-values
\[
  P^{(k)}(\bm Z, \bm W) = \sup_{\pi^{(k)} \in \Pi^{(k)}} P^{(k)}(\bm
  Z, \bm W; \pi^{(k)}),~k=1,2,
\]
where $P^{(k)}(\bm Z, \bm W; \pi^{(k)})$ denote the p-value of the
$k$th CRT under the randomization distribution $\pi^{(k)}$.
Then
\begin{align*}
&\sup_{\pi \in \Pi} \mathbb{P}\left\{ P^{(1)}(\bm Z, \bm W) \leq
  \alpha^{(1)},P^{(2)}(\bm Z, \bm W) \leq \alpha^{(2)}  \right\} \\
\leq \ &  \sup_{\pi \in \Pi} \mathbb{P} \left\{ P^{(1)}(\bm Z, \bm W; \pi^{(1)}) \leq
         \alpha^{(1)},P^{(2)}(\bm Z, \bm W; \pi^{(2)}) \leq
         \alpha^{(2)}  \right\} \\
\leq \ & \alpha^{(1)} \alpha^{(2)}.
\end{align*}

The above argument generalizes the ``knit-product'' structure
identified in \citet{rosenbaum2017general}, which rely on certain
``independent structure'' of permutation groups. In fact, no special
algebraic structures are required in the construction of sequential
CRTs besides nestedness (in the sense of the conditions in
\Cref{prop:nested}).


==> Figures/3_Multiple_CRT.tex <==
\section{Multiple conditional randomization tests}
\label{sec:multiple-crt}


We next show that \eqref{equ:dominance-3} can still hold under a weaker condition than the nested structure of sequential CRTs.
For example,  when $K = 2$, we can allow  $\mathcal{S}^{(1)}_{\bm z}
\subseteq \mathcal{S}^{(2)}_{\bm z}$ for some $\bm z$ but
$\mathcal{S}^{(1)}_{\bm z^{*}} \supseteq \mathcal{S}^{(2)}_{\bm
  z^{*}}$ for another $\bm z^{*} \neq \bm z$. To formalize this result,
for any subset  of the CRTs $\mathcal{J} \subseteq [K]$, we define
the \emph{union}, \emph{refinement} and \emph{coarsening} of their
conditioning sets  as
\[
  \mathcal{R}^{\mathcal{J}} = \bigcup_{k \in \mathcal{J}}
  \mathcal{R}^{(k)}, \quad
  \underline{\mathcal{R}}^{\mathcal{J}} = \left\{ \bigcap_{j \in \mathcal{J}}
    \mathcal{S}_{\bm z}^{(j)} : \bm z \in
    \mathcal{Z}\right\}, \quad \text{and} \quad
  \overline{\mathcal{R}}^{\mathcal{J}} = \left\{\bigcup_{j \in \mathcal{J}}
    \mathcal{S}^{(j)}_{\bm z}: \bm z \in
    \mathcal{Z}\right\}.
\]
Let $\mathcal{G}^{\mathcal{J}}$ be the $\sigma$-algebra generated
by the sets in $\mathcal{R}^{\mathcal{J}}$, so
$\mathcal{G}^{\mathcal{J}} = \sigma\big(\mathcal{R}^{\mathcal{J}} \big).$
Similarly, the refinement and
coarsening $\sigma$-algebras are defined as
$\underline{\mathcal{G}}^{\mathcal{J}} =
\sigma\big(\underline{\mathcal{R}}^{\mathcal{J}} \big)$ and
$\overline{\mathcal{G}}^{\mathcal{J}} =
\sigma\big(\overline{\mathcal{R}}^{\mathcal{J}} \big)$.

\begin{theorem}\label{thm:general-3}
  Suppose the following two
  conditions
  \begin{equation}
    \label{eq:nested}
    \underline{\mathcal{R}}^{\{j,k\}}\subseteq \mathcal{R}^{\{j,k\}},
  \end{equation}
  \begin{equation} \label{eq:cond-indep-3}
    \left( T^{(j)}_{\bm Z}(\bm Z, \bm W)\right)_{j \in \mathcal{J}} \text{ are independent given }
    \underline{\mathcal{G}}^{\mathcal{J}} , \bm W \text{ for
      all }
    \mathcal{J} \subseteq [K].
  \end{equation}
  are satisfied for all $j, k\in [K]$, $j \neq k$. Under  \Cref{assump:randomization}, for any $ \alpha^{(1)},\dotsc,\alpha^{(K)} \in [0,1]$,
  \begin{equation}\label{equ:dominance-conditional-3}
    \begin{split}
      \mathbb{P}\left\{P^{(1)}(\bm Z, \bm W) \leq \alpha^{(1)},\dotsc, P^{(K)}(\bm
      Z, \bm W) \leq \alpha^{(K)} \mid \overline{\mathcal{G}}^{[K]},
      \bm W\right\}
      \leq \prod_{k=1}^{K}\alpha^{(k)}.
    \end{split}
  \end{equation}
  In consequence, \eqref{equ:dominance-3} holds for any $ \alpha^{(1)},\dotsc,\alpha^{(K)} \in [0,1]$.
\end{theorem}
To check if the conditions in \Cref{thm:general-3} are satisfied, we shall consider $K=2$ or $\mathcal{J} = [2].$
In this case, \eqref{eq:nested} is equivalent to  assuming
\begin{equation}\label{equ:ss}
  \mathcal{S}^{(1)}_{\bm z} \cap \mathcal{S}^{(2)}_{\bm z} = \mathcal{S}^{(1)}_{\bm z} \text{ or } \mathcal{S}^{(2)}_{\bm z},\quad  \forall \bm z \in \mathcal{Z}.
\end{equation}
In other words,  we only need $\mathcal{S}^{(1)}_{\bm z} \subseteq \mathcal{S}^{(2)}_{\bm z}$ or $\mathcal{S}^{(1)}_{\bm z} \supseteq \mathcal{S}^{(2)}_{\bm z}$ for every $\bm z \in \mathcal{Z}$.
In sequential CRTs, \eqref{eq:nested} is immediately satisfied since  the refinement of any two partitions  $\mathcal{R}^{(j)}$ and $\mathcal{R}^{(k)}$  is $\underline{\mathcal{R}}^{\{j,k\}} = \mathcal{R}^{(\max(j,k))}.$
When $K=2$, \eqref{eq:cond-indep-3} is equivalent to assuming
\begin{equation}\label{equ:indep_Tz}
  T_{\bm z}^{(1)}(\bm Z, \bm W) \independent T_{\bm
    z}^{(2)}(\bm Z, \bm W) \mid \bm Z \in \mathcal{S}^{(1)}_{\bm
    z} \cap \mathcal{S}^{(2)}_{\bm z}, \bm W, \quad \forall \bm z
  \in \mathcal{Z}.
\end{equation}
In sequential CRTs,  \eqref{equ:indep_Tz} is implied by \Cref{prop:nested}\ref{item:6_2}:
\[ T^{(k)}(\bm Z,  \bm W) \independent \left( T^{(j)}(\bm Z, \bm W) \right)_{j < k}
  \mid \bm Z \in \mathcal{S}_{m}^{(k)}, \bm W
\]
because $T^{(j)}(\bm Z, \bm W)$ is just a
constant given $\bm Z \in \mathcal{S}_{m}^{(k)}$ when $j < k$.
When $K=2$, the main conclusion \eqref{equ:dominance-conditional-3} is
equivalent to saying that
\[
  \mathbb{P}\left\{P^{(1)}(\bm Z, \bm W) \leq \alpha^{(1)}, P^{(2)}(\bm
    Z, \bm W) \leq \alpha^{(2)}         \mid \bm Z \in \mathcal{S}^{(1)}_{\bm
      z} \cup \mathcal{S}^{(2)}_{\bm z}, \bm W\right\} \leq \alpha^{(1)}
  \alpha^{(2)},
\]
for all $\bm z \in \mathcal{Z}$ and $\alpha^{(1)},\alpha^{(2)} \in
[0,1]$. Then, \eqref{equ:dominance-3} is achieved by taking expectation over  $ \mathcal{S}^{(1)}_{\bm
  z} \cup \mathcal{S}^{(2)}_{\bm z}.$
In the following sections, we will see that when it is unclear if the p-values are nearly independent, we can check the conditions \eqref{equ:ss} and  \eqref{equ:indep_Tz} for a pair of CRTs.
Moreover, we can modify the conditioning sets to create CRTs satisfying the conditions in \Cref{prop:nested}.



% The conditions \eqref{eq:nested} and \eqref{eq:cond-indep-3} are
% satisfied for all $j,k \in [K], j \neq k$

% Moreover, \eqref{eq:cond-indep-3} is automatically satisfied if
% $T^{(j)}(\bm z, \bm W)$ does not
% depend on $\bm z$ when $\bm z \in \mathcal{S}_m^{(k)}$ for any $m$ and
% $k>j$. In other words, $T^{(j)}(\bm Z, \bm W)$ is
% $\mathcal{G}^{(k)}$-measurable given $\bm W$ for $j < k$.
% Given this,






























% \Cref{thm:general-3} generalizes this argument by considering the conditioning structure in \eqref{eq:nested}.

% \Cref{prop:nested} generalizes the knit product structure described by
% \citet{rosenbaum2017general}, which essentially requires that
% permutation tests are constructed in a sequential
% manner.




% Following \Cref{def:CRT}, every CRT we consider here is based on a finite or countable partition $\{\mathcal{S}_m\}$ of $\mathcal{Z}$.


% For more discussion and examples, see
% \citet[Sections 3 and 4]{zhang2021multiple_2} and references therein.


==> Figures/4_Example.tex <==

\section{Conditional randomization tests in the literature}
\label{sec:examples}

Next, we apply the general theory in
\Cref{sec:single-crt,sec:multiple-crt} to better understand some
(conditional) randomization tests that have been proposed in the
literature.

\subsection{Permutation tests for treatment effect}
\label{sec:permutation-tests}

Permutation test is the most well known form of conditional
randomization tests. In a permutation test, the p-value is obtained
by calculating all possible values of the test statistics under all
possible permutations of the observed data points. In our setup,
this amounts to use the conditioning sets (suppose $\bm Z$ is a vector
of length $N$)
\begin{equation}
  \label{eq:sz-permutation}
  \mathcal{S}_{\bm z} = \{(z_{\sigma(1)},\dotsc,z_{\sigma(N)}):\text{$\sigma$
    is a permutation of $[N]$}\}.
\end{equation}
In view of \Cref{prop:condition-on-function}, permutation test is a
CRT that conditions on the order statistics of $\bm Z$.
In permutation tests, the treatment assignments are typically assumed
to be exchangeable,
\[
  (Z_1,\dotsc,Z_N) \overset{d}{=} (Z_{\sigma(1)}, \dotsc,
  Z_{\sigma(N)})~\text{for all permutations $\sigma$ of $[N]$},
\]
so each permutation of $\bm Z$ has the same probability of being
realized under the treatment assignment mechanism
$\pi(\cdot)$. See
\cite{kalbfleisch78_likel_method_nonpar_tests} for an alternative
formulation of rank-based tests based on marginal and conditional
likelihoods. Examples of exchangeable assignments include repeated
Bernoulli trials and simple random sampling with or without
replacement (let $Z_i$ be the number of times unit $i$ is
sampled). Exchangeability makes it straightforward to compute the
p-value \eqref{eq:p-value}, as $\bm Z^{*}$ is uniformly distributed
over $\mathcal{S}_{\bm Z}$ if $\bm Z$ has
distinct elements. In this sense, our assumption that the assignment
distribution of $\bm Z$ is known (\Cref{assump:randomization}) is more
general than exchangeability. See \cite{roach2018permutation} for
some recent development on generalized permutation tests in
non-exchangeable models.

Notice that in permutation tests, the invariance of $\mathcal{S}_{\bm
  z}$ in \Cref{lem:same-st} is satisfied because the permutation group
is closed under composition, that is, the composition of two
permutations of $[N]$ is still a permutation of $[N]$. This property
can be violated when the test conditions on additional
events. Southworth et al.\ \cite{southworth2009properties} gives a counterexample in
which $\bm Z$ is randomized uniformly over
\[
  \mathcal{Z} = \{\bm z \in
  \{0,1\}^N: \bm z^T \bm 1 = N/2\},
\]
so exactly half of the units are treated. They consider the ``balanced
permutation test'' in \citep[Section 6]{efron2001empirical} that uses the
following conditioning set
\begin{equation}
  \label{eq:balanced-permutation}
  \mathcal{S}_{\bm z} = \{\bm z^{*}:
  \text{$\bm z^{*}$ is a permutation of $\bm z$ and } \bm z^T \bm z^{*}
  = N/4\}.
\end{equation}
Southworth et al.\ \cite{southworth2009properties} showed that the standard theory
for permutation tests in \citep{lehmann2006testing} does not
establish the validity of the balanced permutation tests, because
$\mathcal{S}_{\bm z}$ is not a group under
balanced permutations (nor is $\mathcal{S}_{\bm z} \cup \{\bm
z\}$). They also provided numerical examples in which
the balanced permutation test has an inflated type I error.

With the general theory in \Cref{sec:single-crt} in mind, we see that
\eqref{eq:balanced-permutation} clearly does not satisfy the
invariance property in \Cref{lem:same-st}. Moreover, a group
structure is not necessary in the construction of a valid
randomization test in \Cref{sec:single-crt}. The crucial algebraic structure is that
$\mathcal{R} = \{\mathcal{S}_{\bm z}:\bm z \in \mathcal{Z}\}$ must be a
partition of $\mathcal{Z}$, or equivalently that the conditioning set
$\mathcal{S}_{\bm z}$ must be defined by an equivalence relation. This
is clearly not satisfied by \eqref{eq:balanced-permutation}.

\subsection{Permutation tests for independence}
\label{sec:tests-cond-indep}

Randomization tests are frequently used to test the independence of random
variables. % In fact, any exact hypothesis test must be a permutation
% test, because the vector of order statistics is a complete suffcient
% statistics; see \citep[Theorem 5.8.1]{lehmann2006testing} or
% \citep[Theorem 3.2.1.1]{hajek1999theory}.
In this problem, it is typically assumed that we observe
independent and identically distributed random variables
$(Z_1,Y_1),\dotsc,(Z_n,Y_n)$ and would like to test the null
hypothesis that $Z_1$ and $Y_1$ are independent. In the classical
treatment of this problem \citep{lehmann2006testing,hajek1999theory},
the key idea is to establish the following \emph{permutation
  principle}:
\[
  (Z_1,\dotsc,Z_N,Y_1,\dotsc,Y_N) \overset{d}{=}
  (Z_{\sigma(1)},\dotsc,Z_{\sigma(N)},Y_1,\dotsc,Y_N)~\text{for all
    permutations $\sigma$ of $[N]$}.
\]
Let $\bm Z = (Z_1, \dotsc, Z_N)$, $\bm Y = (Y_1,\dotsc,Y_N)$, and
$\bm Z_{\sigma} = (Z_{\sigma(1)}, \dotsc, Z_{\sigma(N)})$. Then given
a test statistic $T(\bm Z, \bm Y)$, independence is rejected if the
following p-value is less than the significance level (recall that
there are $N!$ permutations of $[N]$):
\begin{equation}
  \label{eq:p-value-permutation}
  P(\bm Z, \bm Y) = \frac{1}{N!} \sum_{\sigma} 1_{\{T(\bm Z_{\sigma},
    \bm Y) \leq T(\bm Z, \bm Y)\}}.
\end{equation}
We are using the same notation $P(\bm Z, \bm Y)$ for the
p-value of this permutation test in \eqref{eq:p-value-permutation},
because they are indeed identical. It might seem that the permutation
test is solving a different problem
from testing a causal null hypothesis---after all, no
counterfactuals are involved in testing independence. In fact,
Lehmann \cite{lehmann1975nonparametrics} referred to the causal inference
problem as the \emph{randomization model} and the independence testing
problem as the \emph{population
  model}. Ernst \cite{ernst2004permutation} argued that the reasoning
behind these two models is different.

However, a statistical test not only explicitly tests the null hypothesis $H_0$
but also implicitly tests any assumptions needed to set up the
problem. Therefore, the CRT described in \Cref{sec:single-crt} tests
not only a partially sharp null hypothesis about the causal effect
but also the assumption that the treatment is randomized
(\Cref{assump:randomization}). If we simply ``define'' the potential
outcomes as $\bm Y(\bm z) = \bm Y$ for all
$\bm z \in \mathcal{Z}$ so $\bm W$ consists of many identical copies
of $\bm Y$, the ``causal'' null
hypothesis $H_0:\bm  Y(\bm z) =\bm  Y(\bm z^{*}), \forall \bm z, \bm z^{*} \in
\mathcal{Z}$ would be automatically satisfied. Recall that the p-value
\eqref{eq:p-value} of a CRT is given by
\[
  P(\bm Z, \bm W) = \mathbb{P}^{*} \{T_{\bm Z}(\bm Z^{*}, \bm W)
  \leq T_{\bm Z}(\bm Z, \bm W) \mid \bm Z^{*}\in \mathcal{S}_{\bm Z},
  \bm W \},
\]
and suppose the test statistic is given by $T_{\bm z}(\bm z^{*}, \bm
W) = T(\bm z^{*}, \bm Y(\bm z^{*}))$ as in
\Cref{sec:focal-units}. Because of how the potential outcomes schedule
$\bm W$ is defined in this case, the test statistics is
equal to $T(\bm z^{*}, \bm Y)$. Furthermore, the independence of $\bm
Z$ and $\bm Y$ is equivalent to the independence of $\bm Z$ and $\bm
W$. When $\mathcal{S}_{\bm Z}$ is given by
all the permutations of $\bm Z$ as in \eqref{eq:sz-permutation}, $\bm
Z^{*} \mid \bm Z^{*} \in \mathcal{S}_{\bm Z}$ has the same
distribution as $\bm Z_{\sigma}$ where $\sigma$ is a random
permutation. Combining these observations, we see that the permutation
test of independence is identical to the conditional randomization
test of no causal effect.

In summary, the two formulations of permutation (or more broadly,
randomization) tests are unified in our framework. The CRT tests not
only a partially sharp null hypothesis about the potential outcomes
schedule $\bm W$ but also the independence of $\bm Z$ and $\bm W$
(\Cref{assump:randomization}). In the randomization model, $\bm Z
\independent \bm W$ is guaranteed by randomization, so the CRT gives a
test of the causal null hypothesis. In the population model, the causal null
hypothesis about $\bm W$ is automatically satisfied by definition, so
the CRT gives a test of independence. We would like to stress that
such a unification is only a mathematical one; the logic and
philosophy behind the two formulations are fundamentally different. In
the randomization model, inference is justified by the belief that
randomness introduced by the experimenter is exogenous. In the
population model, inference is justified by mathematical assumptions
such as exchangeability of observations. See \Cref{sec:discussion} for
further discussion.


% \qzz{}{We note that it is popular to use permutation tests for testing independence without specifying any experimenter randomness. In this case, the experimenter is usually assumed to be the nature that randomly chooses the order of $(Z_1,Y_1),\dotsc,(Z_n,Y_n)$ with equal probability in the data generating process. This means that the first two kinds of randomnesses we define in \Cref{new_intro} come from the same source. Experimenter randomnesses for testing causal null hypotheses, e.g.,  some physical acts, are clearly known by analysts. This is in contrast with assuming the random variables are i.i.d. or exchangeable, which is only a conceptualization or approximation of the reality.

% In general, if a CRT is based on an assignment distribution with an approximate or proxy density function $\hat{\pi}(\bm z)$
% instead of the true density function $\pi(\bm z)$, its type-I error guarantee is inflated as $\mathbb{P}\{P\leq \alpha\} \leq \alpha + \|\pi - \hat{\pi} \|_2$.  By viewing the standard assumptions, e.g., i.i.d. or exchangeability, as a special kind of experimenter randomness, we re-emphasize the importance of considering whether they hold or not for a practical problem.
% }

\subsection{Randomization tests for conditional independence}
\label{sec:rand-tests-cond}

Recently, there has been a growing interest in randomization tests for
conditional independence
\citep{candes2018panning,tansey2018holdout,berrett2020conditional,katsevich2020theoretical,liu2020fast}. Similar
to the last section, it is assumed that we observe independent and
identically distributed  random variables $(Z_1,Y_1,X_1),\dotsc,(Z_n,Y_n,X_n)$ and would like the
test $Z_1 \independent Y_1 \mid X_1$. This can be easily incorporated
in our framework by treating $\bm X = (X_1,\dotsc, X_n)$ as fixed; see
the last paragraph in \Cref{sec:potent-outc-fram}. In this case, the
randomization distribution of $\bm Z = (Z_1,\dotsc,Z_n)$ is given by
the conditional distribution of $\bm Z$ of $\bm X$. The same
randomization test can then be applied; see \citep[Section
4.1]{candes2018panning} for more
detail. Berrett et al.\ \cite{berrett2020conditional} extended this test by further
conditioning on the order statistics of $\bm Z$, resulting in a
permutation test.

As a remark on the terminology, the test in the last paragraph was
called ``conditional randomization test'' by
Cand{\`e}s et al.\ \cite{candes2018panning}, because the procedure conditions on $\bm
X$. However, such a conditioning is fundamentally different from
the post-experimental conditioning on $\mathcal{S}_{\bm Z}$, which we
use to distinguish conditional randomization tests from unconditional
ones. When $\bm Z$ is randomized according to $\bm X$,
conditioning on $\bm X$ is obligatory in randomization inference
because it needs to use the randomness introduced by the
experimenter (which is conditional on $\bm X$). On the other hand,
further conditioning on $\mathcal{S}_{\bm Z}$ (or on $g(\bm Z)$ as in
\Cref{prop:condition-on-function}) can be introduced by the analyst to
improve the power or make the p-value computable. For this reason, we
advocate reserving the terminology ``conditional randomization test''
for the latter case.


\subsection{Covariate imbalance and rerandomization}
\label{sec:form-part-covar}

Morgan and Rubin \cite{morgan2012rerandomization} proposed to use rerandomization to
improve covariate balance in experiments and regenerated some interest
in randomization inference
\citep{ding2015randomization,banerjee2017decision,heckman2019perry}. They
recounted a conversation
between Cochran and Fisher, in which Fisher advised to rerandomize if
some baseline covariates are not well balanced by the randomly chosen
assignment. The key insight of
Morgan and Rubin \cite{morgan2012rerandomization} is that the experiment should then
be analyzed with the rerandomization taken into account. More
specifically, rerandomization is simply a rejection sampling algorithm
for randomly choosing $\bm Z$ from
\[
  \mathcal{Z} = \{\bm z: g(\bm z) \leq \eta\},
\]
where $g(\bm z)$ measures the covariate imbalance implied by the
treatment assignment $\bm z$ and $\eta$ is the experimenter's level of
tolerance. Therefore, we simply need to use the randomization
distribution over $\mathcal{Z}$ to carry out the randomization
test. This provides an excellent example for our \emph{main thesis}
that randomization inference should be based exactly on the
randomization introduced by the experimenter and the analyst.

Another way to deal with unlucky draws of treatment assignment is to
condition on the covariate imbalance $g(\bm Z)$
\citep{hennessy2016conditional}. This inspires our
\Cref{prop:condition-on-function} in \Cref{sec:conditioning-sets}. In
our terminology, this is a conditional randomization test because the
analyst has the liberty to choose which function $g(\bm Z)$ to
condition on. On the other hand, the randomization test proposed by
Morgan and Rubin \cite{morgan2012rerandomization} is unconditional.



\subsection{Interference}
\label{sec:interference}

Much of our theoretical development in \Cref{sec:single-crt} is
inspired by an exploding literature on causal inference with
interference
\citep{hudgens2008towards,bowers2013reasoning,aronow2017estimating,athey2018exact,li2019randomization,basse2019randomization,puelz2019graph}. The
key challenge with interference is that not all potential
outcomes are imputable. This can be tackled by conditioning on a
smaller set of treatment assignments, as illustrated in
\Cref{sec:focal-units,sec:bipartite-cliques}. Many methods in this
literature
can be regarded as innovative usage of the general theory
outlined in \Cref{sec:single-crt}. In particular, null hypotheses
commonly have the level-set structure as described in
\Cref{def:level-set}, which simplifies the construction of CRT
significantly. % \textcite{basse2019randomization} appear to be the
% first who attempt to establish a general structure for a single
% CRT.

\subsection{Evidence factors for observational studies}
\label{sec:evidence-factors}

So far our discussion has been focused on randomized experiments, but
the same theory also applies to randomization inference for
observational studies \citep{rosenbaum2002observational}. Many
observational studies are analyzed under the \emph{ignorability}
or \emph{no unmeasured confounders} assumption that the treatment is
randomly assigned after conditioning
on some covariates $\bm X$. In our notation, this means that $\bm Z
\independent \bm W \mid \bm X$. However, the distribution of $\bm Z$
given $\bm X$ (often called the \emph{propensity score}) is typically
unknown and needs to be estimated \citep{rosenbaum1983central}.

Alternatively, one can match the treated units with control units to
recreate a paired or blocked randomized experiment. In the simplest
setup with a binary treatment and pair matching, each pair has one
treated unit and one control unit, but they have exactly the same
covariates. So the treatment vector
can be written as $\bm Z =(Z_{1},\dotsc,Z_{N})$ (suppose $N$ is
even) and is supported on
\[
  \mathcal{Z} = \left\{\bm z \in
    \{0,1\}^N:z_1 + z_2 = 1, \dotsc, z_{N-1} + z_{N} = 1\right\}.
\]
Typically, it is assumed that $\bm Z$ is uniformly distributed
over $\mathcal{Z}$, and a randomization test can be conducted in a
straightforward way by permuting the treatment assignments within the
pairs. The uniform distribution over $\mathcal{Z}$ can be justified by, for
example, assuming the distribution of $Z_i$ only depends on $X_i$
and are independent across $i$ \citep[Section
3.2]{rosenbaum2002observational}.\footnote{In practice, units within a pair are
not always exactly matched, which complicates the randomization
inference \citep[Section 3.6]{rosenbaum2002observational}; see also
\citep{abadie2006large} from the perspective of large sample
properties of the matching estimator of average treatment
effect. Another complication being omitted here is that the matched sets are
typically constructed from a larger set of units. The
standard permutation test can be regarded as a CRT that conditions on
$\mathcal{Z}$. However, our general theory in \Cref{sec:single-crt}
may be inapplicable because $\mathcal{Z}$ depends on treatment
variables of a larger set of units and may not induce a partition. To our
knowledge, this subtle issue has not been acknowledged in the
literature yet.}

When there are concerns about unmeasured confounders,
Rosenbaum \cite{rosenbaum1987sensitivity,rosenbaum2002observational}
introduces a general sensitivity analysis framework of the
ignorability assumption. In essence, Rosenbaum's sensitivity model
allows the distribution $\bm Z$ to be non-uniform over $\mathcal{Z}$,
but the ``degree'' of non-uniformness is bounded. More specifically,
it assumes that
\begin{equation}
  \label{eq:rosenbaum-model}
  \frac{1}{1 + \Gamma} \leq \mathbb{P}(Z_i = 1) \leq \frac{\Gamma}{1 +
    \Gamma},~i = 1,\dotsc,N,
\end{equation}
where $\Gamma \geq 1$ is chosen by the analyst.

Let $\Pi$ be the set of distributions of $\bm Z$ that satisfy
\eqref{eq:rosenbaum-model}. We denote the p-value in
\eqref{eq:p-value} as $P(\bm Z, \bm Y; \pi)$ to emphasize that it
depends on the unknown randomization distribution $\pi$ of
$\bm Z$. For simplicity, we will assume that the p-value
is always computable when discussing sensitivity analysis. Because
each p-value $P(\bm Z, \bm Y; \pi)$ satisfies
\eqref{eq:stoc-domi-marginal} under the null hypothesis if $\pi$ is
indeed the distribution of $\bm Z$, by applying the union bound,
\begin{equation}
  \label{eq:sensitivity-p-value}
  P(\bm Z, \bm Y) = \sup_{\pi \in \Pi} P(\bm Z, \bm Y; \pi)
\end{equation}
satisfies \eqref{eq:stoc-domi-marginal} (stochastically dominates the
uniform distribution over $[0,1]$) if the actual distribution of $\bm
Z$ is indeed in
$\Pi$. Rosenbaum \cite{rosenbaum1987sensitivity,rosenbaum2002observational}
provides analytical solutions to the optimization problem in
\eqref{eq:sensitivity-p-value} for a class of sign-score statistics.

In subsequent works, Rosenbaum
\cite{rosenbaum2010evidence,rosenbaum2011some,rosenbaum2017general}
introduces a concept for observational
studies called ``evidence factors''. This is closely related to our
theory of multiple CRTs in
\Cref{sec:multiple-crt}. Loosely speaking, a causal theory can usually
be represented by several hypotheses. For example, the conclusion
``smoking does not cause lung cancer'' entails at least two
hypotheses: whether or not a person smokes does not alter the risk of
lung cancer, and given that the person smokes, the amount of
cigarettes he or she smokes does not alter the risk of lung cancer
either. Therefore, we can then reject null causal theory if either
hypothesis is rejected. When there are concerns about unmeasured
confounders, we may represent the evidence factors by the p-values
obtained from suitable sensitivity analyses. This typically requires
us to specify a sensitivity model $\Pi$ for each hypothesis and
computing the upper bound in \eqref{eq:sensitivity-p-value}.

Rosenbaum's key observation is that in certain problems, these
evidence factors (p-value upper bounds) are ``independent'' in the sense that they satisfy \eqref{equ:dominance-3} when all the null
hypotheses are true. This allows one to test the global null
and the partial conjunction hypotheses using standard methods
\citep{karmakar2019integrating}. Rosenbaum \cite{rosenbaum2010evidence,rosenbaum2011some}
provides some concrete examples of evidence factors, which essentially
correspond to the sequential CRTs described in \Cref{sec:sequential-crts}.

Rosenbaum \cite{rosenbaum2017general} demonstrates that the permutation
groups of a general class of ``independent'' evidence factors have a
knit product structure. Similar to our remark on Southworth et al.\
\cite{southworth2009properties}
in \Cref{sec:permutation-tests}, we believe that the requirement that
$\mathcal{Z}$ is a group or has a knit product structure is not
necessary. Instead, the key is to construct sequential CRTs that
satisfy the conditions in \Cref{prop:nested}. Because the conditions
in \Cref{prop:nested} do not rely on the distribution of $\bm Z$,
the key stochastic dominance result \eqref{equ:dominance-3} holds for
the p-values $P^{(1)}(\bm Z, \bm Y; \pi), \dotsc, P^{(K)}(\bm Z, \bm
Y; \pi)$ for any distribution $\pi$ of $\bm Z$. By computing the
p-value suprema as in \eqref{eq:sensitivity-p-value}, we see that the
evidence factors satisfy the same stochastic dominance result if the sensitivity model is correct.

\subsection{Conformal prediction}
\label{sec:conformal-prediction}

Conformal prediction is another topic related to randomization
inference that is receiving growing interest in statistics and machine learning
\citep{vovk2005algorithmic,shafer2008tutorial,lei13distribution,lei18distribution}. Consider
a typical regression problem where the data points
$(X_1,Y_1),\dotsc,(X_{N},Y_{N})$ are drawn exchangeably from the same
distribution and $Y_N$ is unobserved. We would like to construct a
prediction interval $\hat{\mathcal{C}}(X_N)$ for the next observation
$(X_N,Y_N)$ such that
\[
  \mathbb{P}(Y_N \in \hat{\mathcal{C}}(X_N)) \leq 1 - \alpha.
\]
The key idea of conformal inference is that the exchangeability of
$(X_1,Y_1),\dotsc, (X_N,Y_N)$ allows us to
test the null hypothesis $H_0:Y_N = y$ using permutation tests. More
concretely, we may fit \emph{any} regression model to
$(X_1,Y_1),\dotsc,(X_{N-1},Y_{N-1}),(X_N,y)$ and let the p-value be
one minus the percentile of the absolute residual of $(X_N,y)$ among
all $N$ absolute regression residuals. Intuitively, a large
residual of $(X_N,y)$ indicates that the prediction $(X_N,y)$
``conforms'' poorly with the other observations, so $H_0:Y_N = y$ should be
rejected.

We argue that conformal prediction is a special instance of
the randomization inference described in \Cref{sec:single-crt}. The
key idea is to view random sampling as a
kind of randomization. Notice that conformal prediction implicitly
conditions on the unordered data points $(X_1,Y_1),\dotsc,(X_N,Y_N)$. To
make this more explicit, let the treatment variable $Z$ be the
order of the observations, which is a random permutation of $[N]$ or
equivalently a random bijection from $[N]$ to $[N]$. The
``potential outcomes'' are given by
\begin{equation}
  \label{eq:conformal-counterfactual}
  \bm Y(z)  = \left( (X_{z(1)},Y_{z(1)}),\dotsc,(X_{z(N)},Y_{z(N)}) \right),
%  \begin{cases}
%    (X_{z(i)}, Y_{z(i)}), & \text{if}~i=1,\dotsc,N-1, \\
%    X_{z(N)}, & \text{if}~i=N,
%  \end{cases}
\end{equation}
where $Y_{z(N)}$ is unobserved (that is, the observed $\bm Y$ is the
first $2N-1$ elements of $\bm Y(\bm Z)$). The notation $\bm Y$ is
overloaded here to be consistent with \Cref{sec:single-crt}. The
``potential outcomes schedule'' in our setup is
$\bm W = \left\{\bm Y(z) : \text{ $z$ is a permutation of $[N]$}\right\}$.

The null hypothesis in conformal prediction can be represented
as a regression model $f(x)$ such that the missing $Y_{z(N)}$ is imputed by
$f(X_{z(N)})$. This is a sharp null hypothesis and our theory in
\Cref{sec:single-crt} can be directly used to construct a
randomization test. Notice that the key randomization assumption $Z
\independent \bm W$ in our theory (\Cref{assump:randomization}) is
justified here by the assumption that $(X_1,Y_1),\dotsc,(X_N,Y_N)$ are
exchangeable. In other words, we may view random sampling as a form of
randomizing the order of the observations.

The above argument can be extended to allow ``covariate shift'' in the
next observation $X_N$
\citep{tibshirani2019conformal,hu20distribution}. The key idea is,
again, to consider the randomization involved in sampling. For this we need
to consider a (potentially infinite) super-population $(X_i,Y_i)_{i
  \in \mathcal{I}}$. The ``treatment'' $Z: [N] \to \mathcal{I}$
selects which units are observed. For example, $Z(1) = i$ means that
$(X_i,Y_i)$ is the first data point. The ``potential outcomes'' are still
given by \eqref{eq:conformal-counterfactual}. By conditioning on
unordered $Z$, we can obtain a conditional randomization test
for the unobserved $Y_{z(N)}$. Covariate shift in $X_N$ can be easily
incorporated by conditioning on $(X_{Z(1)},\dotsc, X_{Z(N)})$ and deriving the
conditional distribution of $Z$. For
example, suppose the first $N-1$ units
are sampled from the population according to a covariate distribution
$\pi_1(\bm x)$ and the last unit is sampled according to another
covariate distribution $\pi_2(\bm x)$, that is,
\begin{equation}
  \label{eq:cov-shift-dist}
  \begin{split}
  &\mathbb{P}(Z(k) = i) \propto \pi_1(X_i)~\text{for}~k=1,\dotsc,N-1,i \in
  \mathcal{I}, \\
  &\mathbb{P}(Z(N) = i) \propto \pi_2(X_i)~\text{for}~i \in
  \mathcal{I}.
  \end{split}
\end{equation}
For simplicity, we assume the data points are sampled without
replacement. Then the unordered $Z= \{Z(1),\dotsc,Z(N)\}$ is a set
$\mathcal{S} = \{s_1,\dotsc,s_N\}$ of $N$ distinct units. Let $\bm X =
(X_{s_1},\dotsc,X_{s_N})$. The conditional randomization
distribution of $Z$ is given by
\begin{align*}
  \P\left(Z(N) = s_i \mid \bm X, \mathcal{S}\right)
  % &
    \propto % \sum_{z:z(N)=s_i }
      \pi_2(X_{z(N)})  \prod_{j =1}^{N-1}\pi_1(X_{z(j)})         % \\
 % &= \frac{\pi_2(X_{s_i})q(Y_{s_i}\mid X_{s_i})}{\pi_1(X_{s_i})q(Y_{s_i}\mid X_{s_i})}\sum_{z:z(N)=s_i } \prod_{j =1}^{N}\pi_1(X_{z(j)})q(Y_{z(j)}\mid X_{z(j)})\\
 % &
   \propto \frac{\pi_2(X_{s_i})}{\pi_1(X_{s_i})},~i=1,\dotsc,N,
\end{align*}
by using the fact that the product $\prod_{j=1}^{N}\pi_1(X_{z(j)}) =
\prod_{j=1}^N$ $\pi_1(X_{s_j})$ only depends on $\mathcal{S}$.
By normalizing the probabilities, we obtain
\[
  \P\left(Z(N) = s_i \mid \bm X,\mathcal{S}\right)
  =
  \frac{\pi_2(X_{s_i})/\pi_1(X_{s_i})}{\sum_{j=1}^N\pi_2(X_{s_j})/\pi_1(X_{s_j})},~ i=1,\dotsc,N.
\]
% The same result holds if one further includes a common term $q(Y_i
% \mid X_i)$ ($q(Y \mid X)$ can be any conditional density function of $Y$ given $X$) in the
% randomization distributions \eqref{eq:cov-shift-dist} and conditions
% on the data points $(X_{s_1},Y_{s_1}),\dotsc, (X_{s_N},Y_{s_N})$, as the common term $\prod_{j=1}^N
% q(Y_{s_j}\mid X_{s_j})$ is cancelled during normalization.

The last display equation was termed ``weighted exchangeability'' in
\cite{tibshirani2019conformal}. Again, we would like to stress
that exchangeability (unweighted or weighted) is not necessary
here. What is necessary is a careful consideration of the
randomization $\bm Z$ in the problem. This could be
either explicit as in a physical intervention, or implicit as in
random sampling. Once the randomization distribution of $\bm Z$ is
given and a suitable conditioning set $\mathcal{S}_{\bm Z}$ is found,
the rest is just a straightforward application of the general
conditional randomization test. For example, sampling schemes that are
more general than \eqref{eq:cov-shift-dist} can in principle be
allowed, although the conditional randomization distribution might not
be as simple as above.




==> Figures/5_Applications.tex <==
\section{Application 2: Stepped-wedge trials} \label{sec:swd}

%We next demonstrate the versatility of our theory using the
%stepped-wedge randomized controlled trials, Following our theory, we develop a method
%(\Cref{alg:mcrts}) to construct nearly independent CRTs for lagged
%treatment effects in \Cref{sec:sw-nested-crts}. We also consider
%methods to combine the tests in \Cref{sec:combine}.

%\subsection{Hypotheses for lagged treatment effect}

As introduced in \Cref{label:s_exp}, in stepped-wedge randomized
trials the cross-over time of a unit/cluster from control to treatment
is randomized. This presents a unique opportunity to study how fast
the treatment effect ``kicks in'' by using sequential CRTs.
For simplicity, we assume in this section that the
cross-over times are randomized at the unit level. Our method applies
to cluster-randomized trials by using aggregated cluster-level outcomes
\citep{middleton2015unbiased,thompson2018robust}.



Consider a stepped-wedge trial on $N$ units over some evenly spaced time
grid $[T] = \{1,\cdots,T\}$. At time $t$, a total of $N_t \geq 0$ units
cross-over from control to treatment, and for simplicity we assume
$\sum_{t=1}^T N_t = N$ so all units are treated when the trial is
finished. The cross-overs can be represented
by a binary $N \times T$ matrix $\bm Z$, where $Z_{it} =
1$ indicates that unit $i$ crosses over from control to treatment at time $t$.
We consider the simple scenario of ``complete randomization'', where
$\bm Z$ is uniform assigned over
  $\mathcal{Z} = \left\{\bm z \in \{0,1\}^{N\times T}: \bm
    z\bm 1 = \bm 1, \bm 1^{\top} \bm z  = (N_1,\cdots,N_T)\right\}$.
Thus, the treatment assignment mechanism is given by $\pi(\bm z) = 1 / |\mathcal{Z}|$ where 
$|\mathcal{Z}| = N! / (N_1! \dotsc N_T!)$.  

After the cross-overs at time $t$, we assume the experimenter
immediately measures the outcomes of all units, denoted by
$\bm Y_t \in \mathbb{R}^N$. The corresponding vector of potential
outcomes under the assignments $\bm Z = \bm z$ is denoted by $\bm
Y_t(\bm z) = (Y_{1t}(\bm z), \dotsc, Y_{nt}(\bm z))$. Let $\bm Y =
(\bm Y_1,\dotsc, \bm Y_T)$ be all the realized outcomes and $\bm Y(\bm z)$ be the
collection of potential outcomes under treatment assignment $\bm z \in
\mathcal{Z}$. As usual, we assume the observed outcomes are consistent,
$\bm Y = \bm Y(\bm Z)$.

In this setting, several previous articles have developed
undconditional randomization tests  for the null hypothesis of no treatment
effect whatsoever \citep{ji2017randomization,
  wang2017use, hughes2020rob}, that is,
\begin{equation}
  \label{eq:swd-sharp-null}
  H: \bm Y(\bm z) = \bm Y(\bm z^{*}),\quad \forall \bm z, \bm z^{*} \in
  \mathcal{Z}, i \in [N], \text{ and } t\in [T].
\end{equation}
But as discussed in the introduction,  $H$ is a rather restrictive
hypothesis. Next, we formulate CRTs that test a sequence of hypotheses
about lagged treatment effects.

% We can understand the treatment effects more precisely by
% testing the hypotheses of lagged effects. As the sub-hypotheses of
% $H$, they can show us how soon the treatment effect takes place and
% fades away over time.


\subsection{Testing lagged treatment effect}
\label{sec:sw-nested-crts}

To make the problem more tractable, we assume no interference between
units and no anticipation effect from treatment assigned in the
future; see \citet{athey2018design} for discussion on these
assumptions.

\begin{assumption}\label{assumption:noanti}
  For all $i\in [N]$ and $t\in[T]$, $Y_{it}(\bm z)$ only depends on $\bm
  z$ through $\bm z_{i,[t]}$, the history of  treatment for unit $i$
  up to time $t$.
\end{assumption}

Under this assumption, we may write the potential outcome as
$Y_{it}(\bm z_{i,[t]})$.

Consider a fixed time lag $l$ between $0$ and $T-1$ and the following
sequence of hypotheses about treatment effect of lag $l$:
for $t = 1,\dotsc,T-l$,
\begin{equation}\label{equ:null_st}
  H^{(t)}: Y_{i,t+l}((\bm 0_{t-1},1,\bm 0_{l}))- Y_{i,t+l}(\bm 0_{t+l}) = \tau_{l},\ \forall i\in [N].
\end{equation}
In words, $H^{(t)}$ means that crossing over at time $t$ has a constant
treatment effect $\tau_l$ on the outcome at time $t+l$.

Next, we construct a squence of CRTs for $H^{(1)},\dotsc,H^{(T-l)}$,
which can be combined to test their intersection, which is still much
weaker than the fully sharp null $H$ above. It can not be tested by a
single (conditional) randomization test (CRT). Such a test needs to
compare outcomes across all time steps. Before we proceed, note that
it is impossible to form a single CRT for the intersection null
hypothesis because the hypothesis is not strong enough to impute all
relevant potential outcomes.

% Each $H^{(t)}$ can only impute the control outcomes $Y_{i,t+l}(\bm 0_{t+l})$ and the outcomes $Y_{i,t+l}((\bm 0_{t-1},1,\bm 0_{l}))$ treated exactly $l$ steps ago.
% If under $\bm z^{*}$, a unit crosses over at a time different from $\bm Z$, then all its treated outcomes (except the one treated  $l$ steps ago)  are non-imputable.

% We next consider testing each hypothesis $H^{(t)}$ via a CRT and then combine the p-values to test the intersection.
Observe that in \eqref{equ:null_st}, $H^{(t)}$ only concerns the
potential outcomes of  $Y_{i,t+l}$ when cross-over occurs at time $t$
or after $t+l$. Thus, to test $H^{(t)}$ a natural idea is to compare
units who cross-over at $t$ with those who cross-over after
$t+l$. In other words, we condition on
\begin{equation}
  \label{eq:swd-naive-conditioning}
  g^{(t)}(\bm Z) = \left\{i \in [N]: \bm Z_{i,[t+l]} = (\bm 0_{t-1},1,\bm  0_{l}) \text{ or } \bm 0_{t+l} \right\},
\end{equation}
For any unit $i \in g^{(t)}(\bm Z)$, one of the two potential outcomes
$Y_{i,t+l}((\bm 0_{t-1},1,\bm 0_{l}))$ and $Y_{i,t+l}(\bm 0_{t+l})$
is observed and the other one can easily be imputed from
$H^{(t)}$. Following the construction in \Cref{sec:single-crt}, we can
the easily construct a CRT for $H^{(t)}$. The p-value of this test is
comptuable if the test statistic only depends on the imputable
potential outcomes. For example, we may take the test statistic to be
the average difference between the potential outcomes $Y_{i,t+l}((\bm
0_{t-1},1,\bm 0_{l}))$ and $Y_{i,t+l}(\bm 0_{t+l})$ for $i \in
g^{(t)}(\bm Z)$. Since the assignment mechanism $\pi(\cdot)$ is
uniform over $\mathcal{Z}$, the conditional randomization distribution
is uniform over all permutations of units in $g^{(t)}(\bm Z)$, this
CRT is a permutation test.

% Suppose that we want to include unit $i$ and assignment  $\bm z^*$ in the CRT for $H^{(t)}.$ Then we would need unit $i$ to cross over either at time $t$ or after time $t+l$ under both $\bm Z$ and $\bm z^*$.
% In this case, either of the outcomes in \eqref{equ:null_st} is observed under $\bm Z,$ i.e.,
% \[
% Y_{i,t+l} = Y_{i,t+l}((\bm 0_{t-1},1,\bm 0_{l})) \  \text{ or } \ Y_{i,t+l}(\bm 0_{t+l})
% \]
% then we can impute the another one  under $\bm z^*$.
% By no anticipation in \Cref{assumption:noanti}, $Y_{i,t+l} = Y_{i,t+l}(\bm 0_{t+l})$ if unit $i$ crosses over after time $t+l$.
% We define the mapping
% \begin{equation}
%   \label{eq:swd-naive-conditioning}
%   g^{(t)}(\bm Z) = \left\{i \in [N]: \bm Z_{i,[t+l]} = (\bm 0_{t-1},1,\bm  0_{l}) \text{ or } \bm 0_{t+l} \right\},
% \end{equation}
% which records which units that cross over at time $t$ or after time $t+l$ under $\bm Z$.
% Putting together the assignments that give the same value of $g^{(t)}$, we have the conditioning sets of the CRT,
% $\mathcal{S}_{g}^{(t)} =  \big\{\bm{z}^* \in \mathcal{Z}: g^{(t)}(\bm{z}^*) = g  \big\}$ for all possible value $g$ of $g^{(t)}.$
% They  form a finite partition of $\mathcal{Z}$ based on the value of $g^{(t)}$.
% Like in \Cref{def:CRT}, for any $\bm z \in \mathcal{S}_g^{(t)}$,  we let $\mathcal{S}_{\bm z}^{(t)} = \mathcal{S}_g^{(t)}$
% and  $T_{\bm z}(\cdot,\cdot) = T_g(\cdot,\cdot)$.  Furthermore, we let $ T_g$ only depend on the potential outcomes
%  $Y_{i,t+l}((\bm 0_{t-1},1,\bm 0_{l}))$ and $Y_{i,t+l}(\bm 0_{t+l})$ for unit $i\in g.$ They are either equal to or imputable from the observed outcome $Y_{i,t+l}$ for unit $i\in g.$
% Replacing $\bm W$ with $\bm Y$ in  \eqref{eq:p-value},
% we rewrite this computable p-value as
% \[
%     P(\bm Z, \bm Y) = \mathbb{P}^{*} \{T_{\bm Z}(\bm Z^{*}, \bm Y)
%     \leq T_{\bm Z}(\bm Z, \bm Y) \mid \bm Z^{*}\in \mathcal{S}_{\bm Z},
%     \bm Y \},
% \]
% Since the assignment mechanism $\pi(\cdot)$ is uniform over $\mathcal{Z}$, $ \mathbb{P}^{*} \{\cdot\mid \bm Z^{*}\in \mathcal{S}_{\bm Z},\bm Y \}$ is also a uniform distribution over $\mathcal{S}_{\bm Z}$.
% The CRT can be implemented by permuting the outcomes of units that cross over at time $t$ and after time $t+l$.


%
%\[
%\mathcal{S}_{\bm z}^{(t)} =  \big\{\bm{z}^* \in \mathcal{Z}:
%g^{(t)}(\bm{z}^*) =  g^{(t)}(\bm z) \big\}, \forall  \bm{z} \in
%\mathcal{Z},
%\]










%The function $g$ is often known as an
%\emph{exposure mapping} in the causal inference literature\anonymize{
%\citep[see][Section 4 and references therein]{zhang2021multiple_2}}.







%Collecting all the units we can use under $\bm z^*$ when $\bm Z=\bm z$ , We define the imputability mapping of $H^{(t)}$ as
%\[
 % \mathcal{H}^{(t)}(\bm
%z,\bm z^*) = \left\{i \in [N] : \bm z_{i,[t+l]}, \bm z^*_{i,[t+l]} \in \left\{(\bm
%    0_{t-1},1,\bm
%    0_{l}),\bm 0_{t+l}\right\} \right\}.
%\]







%We first note that $H^{(t)}$ is partially sharp. In fact, if we denote the
%imputability mapping of $H^{(t)}$ as $\mathcal{H}^{(t)}(\bm z,\bm
%z^*)$ (see \Cref{def:hypothesis}), (i.e., $i \in \mathcal{H}^{(t)}(\bm z,\bm z^*)$)






%However, a careful examination reveals that the conditioning sets
%$\mathcal{S}_{\bm Z}^{(1)},\dotsc,\mathcal{S}_{\bm Z}^{(T-l)}$ fail to
%satisfy the nested condition \eqref{eq:nested} in \Cref{thm:general-3}
%when lag $l \geq 1$.

\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{\textwidth}  \centering 
    \includegraphics[width = 0.9\textwidth]{./Figures/swd_dependent_v2}
    \caption{Non-nested CRTs.} \label{fig:swd-crt-1}
  \end{subfigure}
  \begin{subfigure}[b]{\textwidth}\centering 
    \includegraphics[width = 0.9\textwidth]{./Figures/swd_independent_v2}
    \caption{Nested CRTs.} \label{fig:swd-crt-2}
  \end{subfigure}
  \caption{Illustration of the CRTs for the lagged treatment effect
    in a stepped-wedge randomized trial with $T = 8$ time points (lag
    $l=1$).}
  \label{fig:swd-crt}
\end{figure}

However, the above construction of individual CRTs does not lead to
nearly independent p-values. We use \Cref{fig:swd-crt-1} to visualize
the problem where the lag is $l=1$. In this case, the CRT for
$H^{(t)}$ is a permutation test that compares the time $t+1$ outcome
of units that
cross over at $t$ with the units that cross over after
$t+1$. Specifically, CRT 1 compares cross-overs at time
$1$ with cross-overs at time $3,4,\dotsc$; CRT 2 compares
cross-overs at time $2$ and cross-overs at time
$4,5\dotsc$; and so on. As every unit can only cross-over once, it is
easy to see that $g^{(1)}(\bm z)$ is not a function of $g^{(2)}(\bm
z)$ and vice versa, so the conditioning events of CRT 1 and CRT 2 are
not nested (i.e.\ do not satisfy condition \ref{item:6_1} in
\Cref{prop:nested}).


% the
% conditioning set of CRT 1 includes crossing over after time 2, which
% is exclusive of crossing over at time 2 in the conditioning set of CRT
% 2.
% This simple example shows that these CRTs are not independent.
% It also echoes our discussion above that no single CRT can be
% constructed to test the intersection of the hypotheses $H^{(t)},
% t=1,\dotsc,T$. Suppose we would like
% to test $H^{(1)} \cap H^{(2)}$ with lag $l=1$. % a statistic of
% % the form $T(\bm Z, \bm Y_2(\bm Z), \bm Y_3(\bm Z))$ that depends on
% %potential outcomes at $t = 2$ and $3$. % This requires us to be able
% % to impute $\bm Y_2(\bm Z^{*})$ and $\bm Y_3(\bm Z^{*})$ at least for
% % some $\bm Z^{*}$.
% Notice that the treated outcome of unit i at time $3$ is
% not imputable if unit i crosses over at time 1
% because the lag of the effect is
% $l=1$ not 2 (see CRT2 in \Cref{fig:swd-crt-1}). The units treated at time $1$
% must be excluded from the test. However, the dilemma is that they are exactly the units which experience lag 1 effect at time 2.

To resolve this problem, we gain some ideas by considering a even simpler case with $l=0$.
Observe that the stepped-wedge trial can be viewed as a sequentially
randomized
experiment: the assignments $\bm Z$ can be thought of as randomly starting the
treatment for $N_t$ untreated units at every $t = 1,\dotsc,T$. More precisely,  let $\bm Z_t$ denote the $t$-th column of $\bm Z$,
$\bm z_{[t]} = (\bm z_1, \dotsc, \bm z_t) \in \{0,1\}^{N \times t}$ and $N_{[t]} = \sum_{s=1}^t
N_s$. We can decompose $\pi$ as
\begin{equation}\label{equ:swd_sequence}
  \frac{N_1! \dotsb N_T!}{N!} =\pi(\bm z) = \pi_1(\bm z_1) \pi_2(\bm z_2 \mid \bm z_1) \dotsb
  \pi_T(\bm z_T \mid \bm z_{[T-1]}),
\end{equation}
where $\pi_t$ is a complete randomization that assigns $N_t$
out of $N - N_{[t-1]}$ units to treatment:
\[\pi_t(\bm z_t \mid \bm z_{[t-1]}) = \frac{N_t! (N - N_{[t]})!}{(N -
    N_{[t-1]})!}, ~\forall \\ \bm{z}_t \in \{0,1\}^{N}
  \text{ such that } (\bm 1_N - \bm z_{[t-1]} \bm 1_{t-1})^T \bm z_t = N_t.
\]
In the case of $l=0$, the conditioning variable $g^{(t)}(\bm Z)$ in
\eqref{eq:swd-naive-conditioning} actually induces nested CRTs: CRT 1
compares cross-overs at time $1$ with cross-overs at time $2,3,\dotsc$;
CRT 2 compares cross-overs at time $2$ with cross-overs at time
$3,4\dotsc$; and so on. Intuitively, the first CRT utilizes the
randomness in $\bm Z_1$, the second CRT utilizes the randomness in
$\bm Z_2$ given $\bm Z_1$, and which is exactly the structure of
sequential CRTs identified in \Cref{sec:sequential-crts}.

%It is easy to see that the conditions in
%\Cref{prop:nested} are satisfied if the $t$-th CRT
%only depends on $\bm Z$ through $\bm Z_t$ given $\bm Z_1,\dotsc,\bm Z_{t-1}$.

This observation inspires us to modify the tests for the $l=1$ case
as follows: CRT 1 compares cross-overs at time $1$ with cross-overs at
time $3,5,\dotsc$; (ii) CRT 2 compares
cross-overs at time $2$ with cross-overs at time
$4,6,\dotsc$; CRT 3 compares cross-overs at
time $3$ and cross-overs at time $5,7,\dotsc$; and so on
(see \Cref{fig:swd-crt-2} for an illustration).

By considering smaller
conditioning sets, the odd tests become a sequence of nested CRTs and so do the even
tests. %Thus, the nesting condition \eqref{eq:nested} in \Cref{thm:general-3} holds.
And because all the CRTs further
condition on $ g(\bm Z)= \left\{i \in [N]: Z_{i,t} = 1 \text{ for some odd $t$} \right\},$
it is not difficult to show that
\begin{equation}\label{equ:odd_even}
(\bm Z_1, \bm Z_3,\dotsc)\independent (\bm Z_2,\bm Z_4,\dotsc) \mid g(\bm Z).
\end{equation}
For every $t$, the $t$-th CRT only depends on $\bm Z$ through $\bm Z_t$ and uses the
randomization distribution of $\bm Z_t$ given $\bm Z_{[t-1]}$ and
$g(\bm Z)$. It is easy to verify that the
odd and even tests are conditionally independent. More formal justification for this independence is deferred  to  \Cref{sec:multiple-crt}.
 The p-values of these modified CRTs can now be combined to test the intersection of
$H^{(1)},\dotsc,H^{(T-1)}$ for lag 1 effect using the standard global
tests such as Fisher's combination method and Stouffer's method.

%and thus satisfy the condition \eqref{eq:cond-indep-3} in \Cref{thm:general-3}. Similarly,
%\eqref{eq:cond-indep-3} also holds for the even tests. Finally, the
%odd tests and the even tests satisfy \eqref{eq:cond-indep-3} due to
%\eqref{equ:odd_even}. Therefore,  the p-values of the modified CRTs
%satisfy \eqref{equ:dominance-3} and can be combined using the standard
%global testing methods.

The main idea in the discussion above is that we can further
restrict the conditioning sets when the most obvious conditioning sets are not
nested. This argument can be easily extended to a longer time lag $l$. When $l=1$,
we have divided $[T]$ into two subsets of cross-over times (odd and
even). To test the
lag $l$ effect for $l > 1$, we can simply increase the gap and divide
$[T]$ into disjoint subsets:
$\mathcal{C}_1 =\{1,l+2,2l+3,\dotsc\},\mathcal{C}_2 =
\{2,l+3,2l+4,\dotsc\},\dotsc$. A formal algorithm for general $l$ is
given in \Cref{alg:mcrts} in \Cref{appendix:randomization} and will be referred to as multiple
conditional randomization tests (MCRTs) in what follows.

%Using the
%same argument as in the $l=1$ case above, we can verify the two key
%conditions in \Cref{thm:general-3}.





\subsection{Real data examples}

We next demonstrate an application of our method on two
real stepped-wedge randomized trials. Trial I was conducted to examine
if a chronic care model was more
effective than usual care in the Netherlands between 2010 and 2012
\citep{muntinga2012implementing}. The study consists of 1,147 frail
older adults in 35 primary care practices.
The primary outcome in the dataset was quality of life measured by a
mental health component score (MCS) in a 12-item Short Form
questionnaire (SF-12). The outcome for each adult was measured at a
baseline time point and every 6 months over the study. The trial
randomly assigned some practices to start the chronic care model every
6 months. We treated each practice as an experimental unit ($N = 35, T
= 5$).

Trial II was a stepped-wedge trial performed over the pain clinics of 17
hospitals to estimate the effectiveness of an intervention in reducing
chronic pain for patients \citep[Chapter 6.4]{twiskanalysis2021}. The
outcome was a pain score from 1 (least pain) and 5 (most pain) and six
measurements were taken over time: one at the baseline and five more
equally spaced over a period of twenty weeks. After each measurement,
intervention was started in a few randomly selected
untreated hospitals. We considered each hospital
as an experimental unit and estimated the lag $0,1,2$ and $3$ effects
using hospital-level average outcomes ($N = 17, T = 6$).

For each dataset, we combine the p-values from MCRTs using Stouffer's
method that use a
weighted sum of z-scores; this will be denoted as MCRTs+Z (see
\Cref{sec:combine} for more detail). We compare it with mixed-effects
models, with and without time fixed effects.
\Cref{fig:real_data} report 90\%-confidence intervals (CIs) of the
lagged treatment effects.




For trial I in \Cref{fig:real_data}(a), the mixed-effects model
without using time fixed effects suggests that the new chronic care
model may improve the quality of life. However, as noted by
\citet[Section
6.3.1]{twiskanalysis2021}, this model fails to take into account the
gradual increase in the quality of life over time, irrespective of the
intervention. In contrast, both the mixed-effect model with time fixed
effects and our method MCRTs+Z show that the treatment effect is not
statistically significant, and MCRTs+Z produced slightly longer
confidence intervals. This gap between mixed-effect models with and
without time fixed effects is even more pronounced in trial II. In
\Cref{fig:real_data}(b), the confidence intervals generated by these
models for the same time lag do not even overlap. MCRTs+Z generated
confidence intervals that roughly lie in between, confirming that the
effectiveness of the intervention appear to increase over time.

In conclusion, the MCRTs method introduced here offers a robust
alternative to existing mixed-effect models in inferring lagged
treatment effects. The CIs of mixed-effects models often heavily
depend on model specification. Their coverage rates can drop
significantly when the models are misspecified, while MCRTs always
has good coverage properties (as it is based on randomization
tests). This is demonstrated by simulations in
\Cref{sect:sim_2_mixed}.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.8\linewidth]{./Figures/exp_real}
  \caption{Effect estimates from MCRTs+Z and mixed-effects models with and without time effect parameters: 90\%-confidence intervals (CIs) of lagged effects on real data collected from four different stepped-wedge randomized trials.}
  \label{fig:real_data}
  \centering
\end{figure}





































































































==> Figures/6_Discussion.tex <==

\section{Discussion}
\label{sec:discussion}

%\Cref{sec:hypothesis-design} shows that partially sharp null hypotheses in complex experimental designs render the classical Fisher randomization tests infeasible for causal inference.
%\Cref{sec:single-crt} addresses this challenge by defining conditional randomization tests (CRTs) with a computable and valid p-values.

In this article, we have developed an overarching theory for understanding
multiple conditional randomization tests and applied it to testing
lagged treatment effects in stepped-wedge randomized trials. A
particularly attractive feature of randomization tests is that they do
not require specifying any models and are thus robust to model
misspecification, which is confirmed in our numerical experiments.

The main theoretical result (\Cref{thm:general-3}) places
no restriction on the assignment mechanism, whether there is
interference, or the nature of the intervention. It provides a general
principle for constructing nearly independent CRTs in complex
experiments. More user-friendly corollaries were provided in
\Cref{sec:how-choose-partition-2}. Sample splitting is another useful
technique when the most obvious CRTs do not satisfy these conditions,
which is employed by our method for the stepped-wedge design in
\Cref{sec:sw-nested-crts}.


In a parallel line of research, it has been shown that a
randomization test with a carefully consutrcted test statistic is
asymptotically valid for testing average treatment effects
\citep{cohen2020gaussian,fogarty2021prepivoted,zhao2021covariate},
``bounded'' null hypotheses \citep{caughey2021randomization}, or
quantiles of individual treatment effects
\citep{caughey2021randomization}. These techniques can be used in
conjunction with our theory to construct nearly independent CRTs beyond
(partially) sharp null hypotheses.

%\begin{comment}
%Besides applications in causal inference, our theory can be useful for
%developing approximation methods for large-scale randomization tests via
%multiple small CRTs. \qz{Anything concrete here? I prefer to not be
%  too speculative about future work.} Following our
%analysis of p-value combination
%methods and the non-asymptotic power analysis for permutation tests in
%\citet{albert2015tests,kim2020minimax}, it is also interesting to
%study under what condition(s), a combination of randomization tests
%has non-trivial power and how to best combine their p-values in finite
%samples.
%\end{comment}
%echoing
%\citet[page F-1]{brillinger1978role} and
%\citet{rubin80comment}, we think randomization test should be viewed as a (if not the most) pristine
%way of inference for a very specific task---testing a (partially) sharp null hypothesis. It is a powerful weapon for statisticians, but certainly not the ultimate weapon. Nevertheless,

==> Figures/7_Experiments.tex <==

\section{Numerical experiments}
\label{sec:experiment}


\subsection{Stepped-wedge design: size and power}

We examine the performance of the MCRTs method in \Cref{sec:swd} by
comparing it with Bonferroni's Method and checking its validity when there are unit-by-time interactions. We let
MCRTs+F and MCRTs+Z denote the combination of MCRTs with Fisher's combination method
\citep{fisher1925statistical} and the Z-score combiner in \Cref{sec:combine}, respectively.
In all the CRTs, we use the difference-in-means statistic and fix the number of permutations to 1000.


As illustrated in \Cref{fig:swd-crt}, the non-nested CRTs have larger
control groups than our nested CRTs created in MCRTs. However, the
non-nested CRTs are not independent and there are limited ways to
combine them. The most widely used method in this case is Bonferroni's
method that rejects the intersection of $K$ hypotheses if the smallest
p-value is less than $\alpha/K$.
One remaining question is whether the reduced sample size in MCRTs
can indeed be compensated by a better p-value combiner. The following simulation
is designed to answer this question empirically by investigating
varying the sample size $N$, trial length $T$, time lag $l$, and
effect sizes $\tau_l$, respectively. We fix $N_1=
\dotsc = N_T = N/T$ and $N_T=N-\sum_{t=1}^{T-1}N_t$ in the stepped-wedge design.
Let $A_i$ to denote the treatment starting
time of unit $i$, i.e., the index of the non-zero entry of $Z_i$.
Outcomes were generated by a linear mixed-effects model,
\[
Y_{it} = \mu_i + 0.5(X_i+t)   + \sum_{l=0}^{T-1}1_{\{A_i-t =l
  \}}\tau_l + \epsilon_{it},~i=1,\dotsc,N,~t=0,\dotsc,T,
\]
where $\mu_i\sim \mathcal N(0,0.25)$, $X_i\sim \mathcal N(0,0.25)$ and
$\epsilon_{it}\sim \mathcal N(0,0.1)$. This assumes that the baseline outcome
$Y_{i0}$ is measured, which is not uncommon in real clinical
trials. Basic parameters were varied in the following ranges: (i)
number of units $N\in \{100,200,300,400,500\}$; (ii) number of time
steps $T\in \{4,6,8,10,12\}$; (iii) time lag $l\in \{0,1,2,3,4\}$;
effect size $\tau_l\in \{0.01,0.02,0.03,0.04,0.05\}$. Empirical
performance of the methods was examined when one of $N$, $T$, and $l$
is changed while the other two are fixed at the medians of their
ranges, respectively. For example, we
increased $N$ from 100 to 500 while keeping $T=8$ and $l=2$. In these
simulations, $\tau_l$ was set to $0$ and $0.03$ to investigate type I
error and power of the methods, respectively.
 One more simulation was created to study the power as the effect size
 $\tau_l$ varies, in which we keep the first three basic parameters at their
 median values $(N=300,T=8, l=2)$ and increase $\tau_l$ from 0.01 to
 0.05. 


\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{./Figures/exp_power}
  \caption{Performance of MCRTs+F, MCRTs+Z and Bonferroni's method: type I error rates and powers in testing lagged effects at five different numbers of units, numbers of time steps, time lags and effect sizes. The results were averaged over 1000 independent runs.}
  \label{fig:error_power}
  \centering
\end{figure}


The upper panels of \Cref{fig:error_power} show that all the methods
control the type I errors at any number of units, time steps and time
lags. The lower panel shows that our methods are more
powerful than Bonferroni's method in all the simulations. MCRTs+Z is
slightly more powerful than MCRTs+F in all experiments. This shows that
the weighted z-score is more effective than Fisher's combination
method for MCRTs. Panels (d) and (g) show that our methods
outperform Bonferroni's method by a wider margin as the sample size or the effect
size increases. Panel (e) establishes the same observation for trial
length, which can be explained by the fixed sample size (so fewer
units start treatment at each step as trial length increases). This is
not an ideal scenario for applying Bonferroni's method, as the
individual tests have diminishing power. Finally,
panel (f) shows that all the methods have smaller power as the lag size increases, and our methods are particularly powerful when the time lag is small. These results are due to facts. First, there are fewer permutation tests available for larger time lags. Moreover, only including the units that are treated after a large time lag,
the control groups in the permutation tests are small.




Overall, these simulations supports the conclusion that that the
sample splitting in MCRTs is a worthy sacrifice as a more powerful
p-value combiner can be applied. Note that every outcome relevant to
lag $l$ effect is still used in at least one tests in
MCRTs. So the reduced sample size in MCRTs may not be as damaging
as it might first appear.




\subsection{Stepped-wedge design: misspecified mixed-effects models }\label{sect:sim_2_mixed}



% Simulation I demonstrates that our methods MCRTs and MCRT+ are
% powerful in testing partially sharp null hypotheses of lagged effects
% by combining multiple permutation tests.
We next investigate the finite-sample properties
of confidence intervals obtained by inverting conditional
randomization tests (see \Cref{appenx:invert} for more details). We compare its efficiency and
robustness with mixed-effects models for estimating lagged
treatment effect.
%\citep{kenny2021analysis}.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.9\linewidth]{./Figures/exp_interact}
  \caption{Performance of MCRTs+F, MCRTs+Z and the mixed-effects model: coverage rates and lengths of confidence intervals (CIs) under the outcome generating processes with no interaction effect and with three different types of covariate-and-time interactions. The results are averaged over 1000 independent runs. }
  \label{fig:interaction}
  \centering
\end{figure}

The treatment generating process was kept
the same as above. Simulation parameters are set as $N=200$,
$T=8$ and lagged effects $(\tau_0,\dotsc,\tau_7) =
(0.1,0.3,0.6,0.4,0.2,0,0,0)$. The treatment effect is gradually realized and then decayed to 0 over time.
%\qz{I think the means that there is an
%  instantaneous ``shock'' effect that gradually dies out. The arguably
%  more realistic setting is $\tau$ increases over time (so treatment
%  effect is gradually realized).
%Could you run some simulations for
%  that as well?}
 For every $i\in [N]$ and $t=0,1,\dotsc,T$, we generate the outcome $Y_{it}$ using a mixed-effects model,
\[
Y_{it} = \mu_i + 0.5(1-0.1\cdot1_{\{m\neq 0\}})(X_i+t) + 0.1 f_m(X_i+t) + \sum_{l=0}^{7}1_{\{A_i-t =l \}}\tau_l+\epsilon_{it},
\]
where $\mu_i\sim \mathcal N(0,0.25)$, $X_i\sim \mathcal N(0,0.25)$,
$\epsilon_{it}\sim \mathcal N(0,0.1)$ and the unit-by-time interaction $f_m(X_i+t)=0$ if $m = 0$ (no interaction),
$(X_i+t)^2$ if $m = 1$ (quadratic interaction), $2\exp[
(X_i+t)/2]$ if $m = 2$ (exponential interaction), and $5\tanh(X_i+t)$
if $m$=3 (hyperbolic tangent interaction).
% \[
% f_m(X_i+t) =
% \begin{cases}
%         0, & \quad \text{if } m = 0,\\
%         (X_i+t)^2, & \quad \text{if } m=1,\\
%         2\exp[ (X_i+t)/2], & \quad \text{if } m=2,\\
% 5\tanh(X_i+t), & \quad \text{if } m=3,
% \end{cases}
% \]
% which correspond, respectively, to no, quadratic, exponential and
% hyperbolic tangent interactions.
We tasked our methods (MCRTs+F and MCRTs+Z) and a mixed-effects model
described below to construct valid
90\%-confidence interval (CIs) for the lagged effects $\tau_0,\dotsc
\tau_4.$ 
%Our methods were implemented in exactly the same way as in
%Simulation I except that the permutation tests were inverted to obtain
%interval estimators. 
The mixed-effects model takes the form
\begin{equation}\label{equ:mixed_model}
Y_{it} = \beta_{0i} + \beta_1 x_i + \beta_2 t +
\sum_{l=0}^{7}\xi_{l}1_{\{A_i-t =l \}}+ \epsilon_{it},
\end{equation}
where $\beta_{0i}$ is a random unit effect, $\beta_1, \beta_2$ are fixed
effects and $\xi_{0},\dotsc,\xi_{7}$ are lagged effects, and were
fitted using the R-package \texttt{lme4}
\citep{Douglas2015bates}. Recently, \citet{kenny2021analysis} proposed mixed-effects models that can leverage the shapes of time-varying treatment effects. Their models are given by specifying some parametric effect curves with the help of basis functions (e.g. cubic spline).
Besides the unit-by-time interaction, the model \eqref{equ:mixed_model} is already correctly specified for modelling the treatment effects and other parts of the outcome generating process above.
Excluding some of the lagged effect parameters $\xi_5,\dotsc,\xi_7$
from the model may change the effect estimates but not the validity of its CIs.

As the unit-by-time interactions are unknown
and fully specifying them would render the model unidentifiable, they
are typically not considered in mixed-effect models. If the stepped-wedge trial is randomized at the cluster levels, one can introduce cluster-by-time interaction effects in a mixed-effects model; see \citep[Equation 3.1]{ji2017randomization} as an example. However, the cluster-by-time interactions are not exactly the same as the interaction between time and some covariates of the units. It depends on if the interaction varies within each cluster and the clusters are defined by the covariates which interact with time.

The upper panels in \Cref{fig:interaction} show that the CIs of the
mixed-effects model only achieve the target coverage rate of $90\%$
for all the lagged effects when there is no unit-by-time interaction
(panel a). In contrast, the CIs
of our methods fulfil the target coverage rate of $90\%$ in all
scenarios. The lower panels show that the valid CIs given by our
methods have reasonable
lengths between 0.05 and 0.10 for covering the true lagged effects
$(\tau_0,\dotsc,\tau_4) = (0.1,0.3,0.6,0.4,0.2)$. Finally, panel
(e) shows that when the linear model is specified correctly,
it gives valid CIs that are narrower than our nonparametric tests.


\subsection{Simulation II: general interference}

We next examine the validity and power of our multiple CRTs method for testing spillover effects in \cref{sect:spillover_range}. We create a completely randomized experiment 
on $N$ units. The simulation parameters are $N\in \{100,150,200,250,300\}$, proportion of treated units $P_N \in \{0.1,0.2,0.3,0.4,0.5\}$ and signal strength $\beta \in \{0,0.5,1.0,1.5,2.0\}$. For $i\in [N],$ unit $i$'s location $\bm X_i = (X_{i1},X_{i2})$ is drawn independently from a mixture of bivariate normal distributions, $X_{i1}\sim 0.5\mathcal{N}(50,100) + 0.3\mathcal{N}(30,56.25) + 0.2 \mathcal{N}(40,56.25) $ and $X_{i2}\sim 0.5\mathcal{N}(50,100) + 0.3\mathcal{N}(60,56.25) + 0.2 \mathcal{N}(20,56.25).$ Let $\bm D$ be the $N\times N$ euclidean distance matrix of the units. The outcome of each unit $i$ is given by
\[
Y_i = 2Z_i +  \sum_{j\in [N]\setminus \{i\}} 1_{\{ \bm D_{ij} \leq ( k-1,k] \}} Z_j \beta \tau_k + E_i,
\]
where  $E_i\sim \mathcal N(0,1)$ and $(\tau_1,\tau_2,\tau_3,\tau_4,\tau_5) = (1.0,0.8,0.6,0.4,0.2)$ is a decreasing spillover effect vector. Like in the previous sections, as we vary one of the parameters  $N,P_N$ and $\beta$, we fix the other two at the median  of their ranges.   In all the CRTs, we use the difference-in-means statistic \eqref{equ:example_statistics_2} and fix the number of permutations at 1000. 


\begin{figure}[h]
% \vspace{4mm}
  \centering
    \includegraphics[width = 0.75\textwidth]{./Figures/over.pdf}
    \caption{Performance of our multiple CRTs method in testing the hypotheses $H^{(k)}$ for $k\in [5]$. The upper panels use the original p-values. The lower panels use the
    combined p-value by Fisher's method. The results are averaged over 1000 independent runs.}
  \label{fig:interference_plot}
\end{figure}
We create the subsets of units  $\mathcal I^{(k)}$, $\mathcal J^{(k)}$ in \eqref{equ:i_j_k} and the hypotheses $H^{(k)}$ in \eqref{equ:spillover_h} by running the sequential covering procedure (illustrated in \Cref{fig:interference_0}) with the interference matrix $\bm B^{(k)} = \big(B_{ij}^{(k)} = 1_{\{ \|\bm X_i - \bm X_j\|_2 \leq k \}}: i,j\in [N]\big)$ for $k\in [5]$. Since  $H^{(k)}$ represents no spillover effect within the distance in  $(k-1,k]$, we can say it also implies $H^{(k+1)},\dotsc,H^{(5)},$ i.e., no spillover effect for distance larger than $k$. Hence, the p-values $P^{(k)},\dotsc, P^{(5)}$ can be combined in testing $H^{(k)}$ via Fisher's method.
In the upper and lower panels of \Cref{fig:interference_plot}, we report the results for testing  $H^{(1)},\dotsc,H^{(5)}$ with the original p-values and combined p-values respectively. 
We can see that in most cases, the power is larger for smaller $k$ except the red curve for $H^{(1)}$. This is because when the sample size or treated proportion is too small, there is a very few units treated within distance 1 then there is no power in rejecting $H^{(1)}$ based on the original p-value. Fortunately, this issue is addressed after combining the p-values $P^{(1)},\dotsc, P^{(5)}$ in panel (d) and (e).
In panel (f), we can see that when the signal strength $\beta=0,$ all the combined p-values control type I error at the desired level $\alpha=0.1$, which verifies that the original p-values are nearly independent as defined in \eqref{equ:dominance-3}.




%Regardless of which method we use, we have fewer data (permutation tests) to estimate the effects at larger time lags, which explain why the lengths of CIs grow with increasing lag sizes.

%Overall, in analyzing stepped-wedge trial data, one can compare the results of mixed-effects models with our methods. If the CIs of the mixed-effects models are not covered by ours, this may hint on that
%the mixed-effects models are misspecified. If covariates information is available in a dataset, we can consider using a semiparametric model to construct the test statistics in our methods, which may give more flexibility and better power in the analysis.










% Trials III and IV were two stepped-wedge randomized trials in the same
% study \citep{haines2017impact} designed to estimate the impacts of
% removing a set of old health
% services and deploying a new set of weekend health service in hospital
% wards, respectively. Although the original
% investigator collected many outcomes to quantify the health impacts,
% we focused on one of the primary outcomes, the patients' (log) length
% of stay in the hospital. We used data collected from the one of the
% two participating hospitals (Dandenong hospital), from which six wards
% participated in the study. Trial III randomly assigned a ward to
% remove the old service every month over 6 months, One month after
% Trial III ended, Trial IV started the new service for one ward every
% month over the next 6 months in the same order as in Trial III.

% As the hospital wards in this study have different medical
% specialities \citep{haines2017impact}, it may be unreasonable to
% directly compare their patients. In other words, randomizing the
% cross-over times of the hospital wards does not provide direct
% evidence on the effectiveness of the intervention on each
% ward. By assuming that the patient admission time were exchangeable
% within each ward and that there was no time effect on the
% length of stay over the duration of the trials, we tested lagged
% treatment effects by permuting patient admission times within the
% wards. Thus, these permutation tests do not
% qualify as a randomization test because they are not based
% on experimental randomization. Using the terminology in
% \citet{zhang2021multiple_2}, they are conditional quasi-randomization
% tests. See \citet[][Section 2]{zhang2021multiple_2} for more
% discussion on the nature of different permutation tests in this same
% example.

% We compared MCRTs+Z with the mixed effect model without a time effect
% parameter. The time effect parameter is non-identifiable in this
% example, because the time variable is given by a linear combination of the indicator variables of the lagged effects.
% See \Cref{appenx:trial_details} for
% more details on the implementation. Results for Trial III and IV are
% shown in panels (c-d) of \Cref{fig:real_data}. Our method (MCRTs+Z) suggests
% that removing the old services increased the log length of stay by
% about 0.2 and there is little evidence that this effect varies over
% time. Our method further shows that the new weekend health service
% might increase the length of stay comparing to no weekend
% service, although the effect, if exists, is likely to be small and
% does not appear to vary with time. These conclusions are in
% discordance with the mixed-effects model,
% which predicts no effects in the first three months of the first
% intervention and progressively negative effect of the second
% intervention. One possible explanation is that the mixed-effect model
% we used may be misspecified.


==> Figures/8_Interference.tex <==
\section{Application 3: Spillover effect under interference} \label{sec:spillover}



As discussed in \Cref{label:c_exp}, estimating spillover effects is crucial for optimizing treatment decisions under unit interference.
Consider a completely randomized experiment on $N$ units.
Suppose that we want to test the spillover effect within a distance $\epsilon$.
We let $\bm D$  denote the $N\times N$ distance matrix of the units.
Thresholding  $\bm D$ by  $\epsilon$, we obtain the interference matrix $\bm B$ of the units.
Denote the observed treatment  assignments by $\bm Z\in \mathcal{Z}\subseteq \{0,1\}^N$.
For every unit $i\in [N]$,  it holds that
\[
Z_i = 0 \text{ and } \bm B_{i}  \bm Z\geq 1 \ \Leftrightarrow  \sum_{j\in [N]\setminus \{i\}} 1_{\{ \bm D_{ij} \leq \epsilon \}} Z_j > 0,
\]
which indicates if unit $i$ is untreated but spillovered by at least one unit in its $\epsilon-$neighbourhood.
To reduce the number of unknown potential outcomes under arbitrary interference,  it is often assumed that $Y_i(\bm z)$ only depends on  $z_i$ and $1_{\{ \bm B_{i}  \bm z \geq 1 \}}.$
\begin{assumption}\label{assumption:interference}
  For any $i\in [N]$ and $\bm z\in \mathcal{Z}$,  $Y_i(\bm z)   = Y_i (z_i, 1_{\{ \bm B_{i}  \bm z \geq 1 \}} ).$
  \end{assumption}
Under \Cref{assumption:interference},  \citet{athey2018exact,puelz2019graph} have proposed methods to test  the following no-spillover-effect hypothesis and its variants:
\[
H_{\epsilon}: Y_i(0,1) = Y_i(0,0) , \forall i\in [N],
\]
which states that there is no difference between being spillovered within the distance $\epsilon$ and control (i.e. being spillovered at any distance larger than $\epsilon$).


In many applications of spillover effects, the treatments (e.g. social policies) often take a considerable amount of resources to assign,
e.g., increasing daily police presence in some streets to reduce the crime rate in Medell\'{i}n \citep{collazos2021hot}. To optimize the treatment allocation, we would need to infer how far the effect can spillover. Testing $H_{\epsilon}$  for a single $\epsilon$  is insufficient for this purpose. When $H_{\epsilon}$ is rejected, it has two implications,  $H_{\epsilon}$ is false or (2) \Cref{assumption:interference} is false. In the case of (2), we only know the spillover effect occurs within any $\delta\epsilon$-neighbourhoods for some $\delta \neq 1$. Testing  $H_{\epsilon}$ for a range of $\epsilon$ is not a straightforward solution. The p-values obtained in this way are mutually dependent and their powers depend heavily on $\epsilon$. When $\epsilon$ is too large, most of the units are regarded as spillovered under \Cref{assumption:interference}. The test for $H_{\epsilon}$ would be powerless. Type I error inflation is inevitable  if we use these p-values selectively, e.g., picking the  $\epsilon$ that attains the smallest p-value.
We next formulate a sequence of nested CRTs and invert their p-values into simultaneously valid confidence intervals to gauge the spillover effect at different distances.

%We note that no matter which method we apply, there is an inherent power problem in testing $H_{\epsilon}$ due to the tradeoff between $\mathcal{I}_{\bm Z}$ and $%\mathcal{S}_{\bm Z}.$ By definition,  the number of never-treated $\mathcal{I}_{\bm Z}$
%decreases as the size of $\mathcal{S}_{\bm Z}$ increases.  In the CRT by \citet{athey2018exact} (with $\bm Z_I^* = \bm Z_I$), as the number of random focals $\mathcal I$ %increases, we have more never-treated units $\mathcal{I}_{\bm Z} = \{i\in \mathcal{I}: Z_i\neq 1 \}$ but less assignments from randomizing $\bm Z_{[N]\setminus I}^{*}.$ %Importantly, the testing power can not be simply explained by  the set sizes $|\mathcal{I}_{\bm Z}|$ and  $|\mathcal{S}_{\bm Z}|.$ A large $\mathcal{S}_{\bm Z}$ may contain %many assignments that are similar to $\bm Z$. The test statistics takes similar values under different values of $\bm Z^*$ so the CRT is powerless.

\subsection{Estimating the range of spillover effect}\label{sect:spillover_range}

To better illustrate our method, we will base our introduction on the forest trial data \citep{jayachandran2017cash} mentioned above.  The experimental units in this dataset are 121 villages in Hoima district and northern Kibaale district in Uganda, 60 of which were randomized to receive the payments annually from 2011 to 2013. The payments should encourage the forest owners to conserve the forests in their villages. However, they may increase deforestation in the nearby untreated villages.   Following the work by \citet{wang2020design}, we use \quotes{the change in land area covered by trees} as our outcome, which is measured from high-resolution satellite images in \citet{hansen2013high}. \Cref{fig:interference_0} (a) shows the units' locations $\bm X = (\bm X_1,\dotsc, \bm X_N)$ in the districts; the distances between most of the units are larger than 3. So we will consider testing if the spillover effect is nonzero between the units whose distances are in $((k-1)\epsilon,k\epsilon]$ for $\epsilon=3$ and $k\in [4]$ respectively.

\begin{figure}[t]
  \centering
    \includegraphics[width = 0.75\textwidth]{./Figures/visual.pdf}
    \caption{A sequential procedure to construct four CRTs in the forest example.}
  \label{fig:interference_0}
\end{figure}

Following the general recipe in \Cref{sec:sequential-crts}, we will divide $\bm Z$ into four components to create four sequential CRTs.
On the basis of this, we will  propose a covering-based method to optimize  the division of $\bm Z$, which makes sure that all CRTs we create are powerful.
We will drop \Cref{assumption:interference}, which implies an unit's outcome is invariant of how many of its neighouring units receive the paytments.
Instead, we assume that the spillover effect from different neighbouring units are cumulative, i.e.,  the incentive to displace deforestation grows as more neighbouring villages receive the payments.

To create a powerful CRT for the spillover effect within the distance $k\epsilon$, we shall consider how to let more units being spillovered within their $k\epsilon$-neighbourhoods (i.e. the $k\epsilon$-balls centred at them).
%We can only optimize the unit selection without looking at the observed assignments $\bm Z$.
%Otherwise, the test will be invalid because its conditioning sets fail to be a partition of the space $\mathcal{Z}.$
We define the interference matrix
$ \bm B^{(k)} = \big(B_{ij}^{(k)} = 1_{\{ \|\bm X_i - \bm X_j\|_2 \leq k\epsilon \}}: i,j\in [N]\big).$
We define the $k\epsilon$-cover of the units as the smallest subset of units whose $k\epsilon$-neighbourhoods together can contain all the units.  Our idea is that by randomizing the assignments of the cover, the other units will have a chance to experience the spillover effect within the distance $k\epsilon.$
Starting from $k=1,$ we let $\mathcal{I}^{[0]} =\emptyset $ and find the minimum set cover
\begin{equation}\label{equ:mini_set}
\mathcal{U}^{(k)} =\argmin_{\mathcal U \subseteq [N]\setminus \mathcal{I}^{[k-1]} } |\mathcal U | \  \text{ subject to } \  \bm B_{i}^{(k)}\bm 1_{\mathcal U} \geq 1, \forall i \in [N]\setminus \mathcal{I}^{[k-1]} .
\end{equation}
The constraint indicates that every unit $i$ is covered by at least one unit in $\mathcal U$. We note that
\eqref{equ:mini_set} is a NP-hard integer linear program. But its linear programming relaxation (LPR) can be solved by a factor-$\log N$ approximation algorithm \citep{vazirani2001approximation}[Chapter 2]; in this paper, we solve it using the function \texttt{setcover} in the R-package \texttt{adagio} \citep{borchers2016adagio}.

When $k$ is small, for some units in the cover, their $k\epsilon$-neighbourhoods only contain themselves so they can not spread the effect to anyone.
This motivates us to refine the subset $\mathcal U^{(k)}$ as $\mathcal{I}^{(k)}$ and then define its $((k-1)\epsilon,k\epsilon]$-neighbours $\mathcal{J}^{(k)} $ as the focal units:
\begin{equation}\label{equ:i_j_k}
\begin{split}
& \mathcal{I}^{(k)} = \left\{i \in \mathcal{U}^{(k)} : \bm B_{i}^{(k)}\bm 1 \geq 2 \right\}  	\\
&  \mathcal{J}^{(k)} = \left\{j \in [N] \setminus \mathcal{I}^{(k)} :  \bm  B_{j}^{(k-1)}\bm 1_{\mathcal{I}^{(k)} } =0, \bm  B_{j}^{(k)}\bm 1_{\mathcal{I}^{(k)} } \geq 1 \right\}.
\end{split}
\end{equation}
As shown in \Cref{fig:interference_0} (b), when $k=1$, the units $\mathcal{I}^{(1)} $ are coloured in red and we will test the effect on its neighbours $\mathcal{J}^{(1)} $ (in green). As $k$ increases to 2,3 and 4,
we let $\mathcal{I}^{[k-1]} := \cup_{b=1}^{k-1} \mathcal{I}^{(b)} $ in \eqref{equ:mini_set} and then repeat the process above to create $\mathcal{I}^{(k)}$ and $ \mathcal{J}^{(k)}$.\footnote{We also remove $\mathcal{I}^{[k-1]} $ in the constraints of \eqref{equ:mini_set}, otherwise, the program may not have a feasible solution, i.e., the neighbourhoods of $[N]\setminus \mathcal{I}^{[k-1]}$ can not cover all the unit $i\in [N].$ }
The subsets $\mathcal{I}^{(k)}$ we find can spread the effect efficiently in the space. By definition, the units $\mathcal{I}^{[k-1]}$ we remove in \eqref{equ:mini_set} still have at least one neighbour remaining in $[N]\setminus \mathcal{I}^{[k-1]}.$ These neighbours are good proxies of $\mathcal{I}^{[k-1]}$. So solving \eqref{equ:mini_set}  with and without $\mathcal{I}^{[k-1]}$ would lead to a similar cover. \Cref{fig:interference_0} (c-e) show that the effect can spillover from $\mathcal{I}^{(k)} $ (in red)  to many other units $\mathcal{J}^{(k)} $ (in green) for $k=2,3,4$;
when $k=1$, the red dots in  \Cref{fig:interference_0} (b) are the only units that can experience a spillover effect within the distance 3. Overall,
by solving a sequence of covering problems, we get to randomize more treatment variables from $\mathcal{I}^{(k)}$'s and use more outcomes from $\mathcal{J}^{(k)}$'s. This makes sure that the CRTs using $\mathcal{I}^{(k)}$'s and $\mathcal{J}^{(k)}$'s are powerful.

Let $\mathcal{I}^{[k]} = \bigcup_{k'\in [k]} \mathcal{I}^{(k')}.$ In our CRTs, we will never randomize (i.e. always condition on) the assignments of the units in $[N]\setminus \mathcal{I}^{[K]}$. To ease the notation, we would assume $\mathcal{I}^{[K] }= [N]$ and omit $[N]\setminus \mathcal{I}^{[K]}$.
Then, we can revoke our notation of sequential CRTs at the end of \Cref{sec:sequential-crts}. Let $\bm Z^{(k)} = \bm Z_{\mathcal{I}^{(k)}}$ and $\bm Z^{(-k)} = \bm Z_{[N]\setminus \mathcal{I}^{(k)}}$ for $k\in [4].$ 
The CRTs we create can be viewed as a sequential clustered randomized experiment. For example of $k=4,$ in  \Cref{fig:interference_0} (e), the (9,12]-neighbourhood of each red unit $i\in \mathcal I^{(4)}$ can be viewed as a cluster. The green units $j\in \mathcal{J}^{(4)}$ in the same neighbourhood shares the same spillover effect. 
Before we proceed, we note that the CRTs for the hypotheses
\[
H_0^{(k)} :\bm Y_{\mathcal{J}^{ (k)}}(\bm z) = \bm  Y_{\mathcal{J}^{ (k)}}(\bm{z}'), \forall \bm z,\bm{z}'\in \mathcal{Z} \text{ s.t. } \bm z^{(-k)} = \bm z'^{(-k)},
\]
are not nested, because the conditioning events $\mathcal{S}_{\bm z}^{(k)} = \{ \bm z^* \in  \mathcal{Z}:     \bm{z}^{*(-k)}= \bm{z}^{(-k)} \}$ for different $k$ fail to satisfy the
first condition in \Cref{prop:nested}. So instead, we consider testing
\begin{equation}\label{equ:spillover_h}
H^{(k)} :\bm Y_{\mathcal{J}^{ (k)}}(\bm z) = \bm  Y_{\mathcal{J}^{ (k)}}(\bm z'), \forall \bm z,\bm z' \in \mathcal{Z} \text{ s.t. } \bm z^{[k-1]} = \bm z'^{[k-1]}.
\end{equation}
where $\mathcal{I}^{[0]} = \emptyset.$
Compared with $H_0^{(k)}$, we no longer fix the assignments $(\bm z^{(k+1)},\dotsc, \bm z^{(K)}).$
For example of $k=1, H^{(1)}$ states that randomizing the assignments of all the red units in \Cref{fig:interference_0} (b-e) makes no difference on the outcomes of the green units  in  \Cref{fig:interference_0} (b).
Arguably, $H_0^{(1)}$ is not much weaker than $H^{(1)}$ because if there is no effect from the nearest neighbours $\mathcal{I}^{(1)}$ to units $\mathcal{J}^{(1)},$ then there is also no effect from units $\mathcal{I}^{(2)}\cup \cdots\cup  \mathcal{I}^{(4)}$ that are further away from units $\mathcal{J}^{(1)}.$
In the CRT for $H^{(k)},$ we let  the test statistics depend on the outcomes of the neighbours $\mathcal{J}^{(k)}$ of units $\mathcal{I}^{(k)}$.
Under  $H^{(k)}$, for any $j\in \mathcal{J}^{(k)}, Y_j(\bm Z^*)$ only depends on  $\bm Z^*$ through $\bm Z^{*[k-1]}.$
Then for all assignments $\bm Z^*$ considered in $H^{(k)},$  we have
\begin{equation}\label{equ:example_statistics_2}
\begin{split}
T^{(k)}  (\bm Z^*, \bm W)  & =  \frac{\sum_{j\in \mathcal{J}^{ (k)}  }  A_j^{(k)}(\bm Z_{\mathcal{I}^{(k)}}^*) Y_j (\bm Z^*)}{      \sum_{i \in \mathcal{J}^{(k)}   }   A_{i}^{(k)}(\bm Z_{\mathcal{I}^{(k)}}^*)    }   -  \frac{\sum_{j'\in \mathcal{J}^{(k)} } \big[1-  A_{j'}^{(k)}(\bm Z_{\mathcal{I}^{(k)}}^*) \big]Y_{j'} (\bm Z^*) }{  \sum_{i' \in \mathcal{J}^{(k)}  }    \big[1-  A_{i'}^{ (k)}(\bm Z_{\mathcal{I}^{(k)}}^*) \big]  }  \\
& =  \frac{\sum_{j\in \mathcal{J}^{ (k)}  }  A_j^{(k)}(\bm Z_{\mathcal{I}^{(k)}}^*) Y_j (\bm Z)}{      \sum_{i \in \mathcal{J}^{(k)}   }   A_{i}^{(k)}(\bm Z_{\mathcal{I}^{(k)}}^*)    }   -  \frac{\sum_{j'\in \mathcal{J}^{(k)} } \big[1-  A_{j'}^{(k)}(\bm Z_{\mathcal{I}^{(k)}}^*) \big]Y_{j'} (\bm Z) }{  \sum_{i' \in \mathcal{J}^{(k)}  }    \big[1-  A_{i'}^{ (k)}(\bm Z_{\mathcal{I}^{(k)}}^*) \big]  }        \\
& \equiv T^{(k)}  (\bm Z^{*[k]}, \bm Y ).
\end{split}
\end{equation}
where $A_j^{(k)}(\bm Z_{\mathcal{I}^{ (k)}}^*)  = 1_{ \big\{ \sum_{u \in \mathcal{I}^{(k)}   }B_{u j}^{(k)} Z_{u}^* \geq 1       \big\}         } $ indicates if the neighbour $j\in \mathcal{J}^{ (k)}$ is spillovered by at least one unit in $\mathcal{I}^{ (k)} $.
We test $H^{(k)}$ using the p-value
\begin{equation}\label{equ:pval_interference}
    P^{ (k)}(\bm Z,\bm Y)   = \mathbb{P}^{*} \big\{ T^{(k)}  (\bm Z^{*[k]}, \bm Y )  \leq T^{(k)}  (\bm Z^{[k]}, \bm Y ) \mid    \bm Z^* \in \mathcal{S}_{\bm Z}^{(k)}  , \bm Y   \big\}.
\end{equation}
where
$\mathcal{S}_{\bm Z}^{(k)} = \big\{ \bm z^* \in \mathcal Z :  \bm z_{*[k-1]} =  \bm Z_{[k-1]}   \big\}.$ The conditioning events and test statistics for all $k\in [K]$ now follow the general construction of sequential CRTs at end of  \Cref{sec:sequential-crts}. Hence, the p-values $P^{ (1)},\dotsc, P^{ (4)}$ are nearly independent as defined in \eqref{equ:dominance-3}.

%Compared with the indicator $1_{ \{ Z_j^* =0, \bm B_{j}  \bm Z^* \geq 1         \}} $ in \eqref{equ:example_statistics},  $A_j^{ (k)}(\bm Z_{\mathcal{I}^{ (k)}}^*) $ only depends on the assignments of $\mathcal{I}^{ (k)} $ but allows the unit $j\in \mathcal{J}^{(k)} $ to be spillovered by other units or even treated directly.
%The partition of our CRT is the collection of subsets $\mathcal{S}_{\bm g}^{ (k)} =  \big\{\bm{z}^* \in \mathcal{Z}: g^{ (k)}(\bm{z}^*) = \bm g  \big\}$ for all value $\bm g$ of $g^{ (k)}.$

Following the preliminary in \Cref{appenx:invert}, we invert these p-values into confidence intervals in \Cref{fig:interference_0} (f). Note that the test statistics $T^{(k)}  (\bm Z_{        \mathcal{I}^{ (k)}}, \bm Y_{\mathcal{J}^{ (k)}})$ only measures the effect from units $\mathcal{I}^{ (k)}$. So we obtain the confidence interval for the constant spillover effect within the interval $(3(k-1),3k]$.The original p-values are 0.035, 0.363, 0.773 and 0.779; see randomization distributions reported in \Cref{fig:interference_3} in \Cref{appendix:randomization}.  In summary, we found that the spillover effect is only significant within 3-neighbourhoods of the treated villages. The payments can encourage more forest conservation near the boundaries of the treated villages, and displacement of deforestation was not a concern for the ecosystem services.

